Online Disjoint Spanning Trees and Polymatroid Bases

Finding the maximum number of disjoint spanning trees in a given graph is a well-studied problem with several applications and connections. The Tutte-Nash-Williams theorem provides a min-max relation for this problem which also extends to disjoint bases in a matroid and leads to efficient algorithms. Several other packing problems such as element disjoint Steiner trees, disjoint set covers, and disjoint dominating sets are NP-Hard but admit an $O(\log n)$-approximation. C\u{a}linescu, Chekuri, and Vondr\'ak viewed all these packing problems as packing bases of a polymatroid and provided a unified perspective. Motivated by applications in wireless networks, recent works have studied the problem of packing set covers in the online model. The online model poses new challenges for packing problems. In particular, it is not clear how to pack a maximum number of disjoint spanning trees in a graph when edges arrive online. Motivated by these applications and theoretical considerations, we formulate an online model for packing bases of a polymatroid, and describe a randomized algorithm with a polylogarithmic competitive ratio. Our algorithm is based on interesting connections to the notion of quotients of a polymatroid that has recently seen applications in polymatroid sparsification. We generalize the previously known result for the online disjoint set cover problem and also address several other packing problems in a unified fashion. For the special case of packing disjoint spanning trees in a graph (or a hypergraph) whose edges arrive online, we provide an alternative to our general algorithm that is simpler and faster while achieving the same poly-logarithmic competitive ratio.

==> introduction-1.tex <==
\section{Introduction}\label{section:intro}

Consider a function $f:2^{\mathcal{N}}\rightarrow \mathbb{R}_{\geq 0}$ on a ground set $\mathcal{N}$ of size $n$. It is \emph{monotone} if $f(A)\leq f(B)$ for every $A\subseteq B$ and \emph{submodular} if $f(A)+f(B)\geq f(A\cup B)+f(A\cap B)$ for every $A,B\subseteq \mathcal{N}$. A subset $S\subseteq \mathcal{N}$ is a \emph{base} of $f$ if $f(S)=f(\mathcal{N})$. A \emph{polymatroid} $f:2^\mathcal{N}\rightarrow \mathbb{Z}_{\geq 0}$ is an integer-valued monotone submodular function with $f(\emptyset)=0$.

In the \emph{Polymatroidal Disjoint Bases} problem, we are given a polymatroid $f:2^{\mathcal{N}}\rightarrow \mathbb{Z}_{\geq 0}$ via an evaluation oracle. The goal is to find a maximum number of disjoint bases. We define $\texttt{Opt}(f):=\max\{k: \exists \ k \text{ disjoint bases of $f$}\}$.

We consider the \emph{Online Polymatroidal Disjoint Bases} problem, where the value $r=f(\mathcal{N})$ is known in advance and the elements $\mathcal{N}$ come in an online fashion. For a color assignment $C:\mathcal{N}\rightarrow \mathbb{Z}_+$, color $c\in \mathbb{Z}_+$ is a \emph{proper color} if the set of elements with color $c$ is a base. An online algorithm has to decide on the color of each element immediately after it arrives, while maximizing the number of proper colors.

Let $\texttt{Alg}(f)$ be the number of proper colors obtained by an online algorithm $\texttt{Alg}$ for a given polymatroid $f$. A deterministic algorithm $\texttt{Alg}$ is \emph{(purely) $\alpha$-competitive} if for every polymatroid $f$, we have
\begin{equation}
    \texttt{Alg}(f)\geq \frac{\texttt{Opt}(f)}{\alpha}. \label{def:competitive-ratio}
\end{equation}
A randomized algorithm is \emph{$\alpha$-competitive} if the bound in (\ref{def:competitive-ratio}) holds in expectation.

In this work, we give an $O(\log^2 r)$-competitive randomized online algorithm for Polymatroidal Disjoint Bases.

\begin{theorem}\label{main-result:polymatroid}
    For the Polymatroidal Disjoint Bases problem, there exists a randomized online algorithm with competitive ratio $O(\log^2 r)$. The algorithm runs in $\mathop{poly}(r, i)$ time when the $i$-th element arrives for every $i\in \mathbb{Z}_+$.
\end{theorem}

We also consider the special case where the given polymatroid $f$ is related to hypergraphs. The input to the problem is a hypergraph $G=(V,E)$ consisting of $n=|V|$ nodes and $m=|E|$ hyperedges, where each hyperedge is a non-empty subset of $V$. For every subset $A\subseteq E$ of hyperedges, let $c(A)$ be the number of connected components in the subhypergraph $(V,A)$ and define $f(A):=n-c(A)$. We can check that $f$ is a polymatroid on $E$ and a base of the polymatroid corresponds to a connected subhypergraph. The goal is to find a color assignment $C: E \rightarrow \mathbb{Z}_+$, which maximizes the number of proper colors $c\in \mathbb{Z}_+$. This problem is called the \emph{Disjoint Connected Spanning Hypergraphs} problem. Theorem~\ref{main-result:polymatroid} implies a randomized online algorithm for this problem with competitive ratio $O(\log^2 n)$. We further show that there is a faster randomized online algorithm with the same competitive ratio.

\begin{theorem}\label{main-result:hypergaph}
    For the Disjoint Connected Spanning Hypergraphs problem, there exists a randomized online algorithm with competitive ratio $O(\log^2 n)$. The algorithm runs in $O(n^2)$ time when each hyperedge arrives.
\end{theorem}

==> proof-algorithm-1.tex <==
\section{An $O(\log^2 r)$-Competitive Algorithm}\label{section:algorithm}
In this section, we present a randomized online algorithm with expected competitive ratio $O(\log^2 r)$ but the run-time of the algorithm at each timestep will be exponential. The purpose of this section is to illustrate that the online arrival order has sufficient information to achieve a reasonable competitive ratio (albeit in exponential runtime) and to highlight the main ideas underlying the eventual polynomial-time algorithm that will prove Theorem \ref{main-result:polymatroid}. %We will modify this algorithm in the Section \ref{section:poly-algorithm} to improve the runtime to polynomial while guaranteeing the same competitive ratio. 
%achieve the same competitive ratio in polynomial time. 
\iffalse
C{\u{a}}linescu, Chekuri, and Vondr\'{a}k \cite{CCV09} showed that if the upper bound $k^*$ is known in advance, then sampling the color of each element $\textit{u.a.r.}$ from $[\lfloor k^*/(\log r + \log\log r) \rfloor]$ leads to an $O(\log r)$-competitive online algorithm. The key challenge in the online setting is the inability to compute $k^*$ without knowing all elements in advance. We will use the minimum sized quotient containing the newly arrived element as the estimate for $k^*$. We show a structural property that at least a constant fraction of elements have their estimate within a $\text{poly}(r)$ factor of $k^*$. We will show that coloring these elements $\textit{u.a.r.}$ from $[\lfloor k^*/\log^2 r \rfloor]$ leads to $\Omega(k^*/\log^2 r)$ proper colors, which implies an $O(\log^2 r)$-competitive online algorithm by the upper bound in Theorem~\ref{thm:CCV-k^*}.
\fi
%We first design an $O(\log^2 r)$ competitive algorithm under the assumption that $r\geq 2$ and $k^*\geq 120\log^2 r$. 
We describe the algorithm in Section~\ref{subsection:algorithm}. We present a novel property of the sequence of minimum sized quotients containing the last element with respect to a fixed ordering in Section~\ref{subsection:property-quotient}. We prove the structural property that 
focusing on elements whose estimates are within a $\text{poly}(r)$ factor of $k^*$ does not decrease $k^*$ by more than a constant factor 
%at least a constant fraction of elements have their estimate within a $\text{poly}(r)$ factor of $k^*$ 
in Section~\ref{subsection:structural-property}. We use these properties to analyze the competitive ratio of the algorithm in Section~\ref{subsection:ratio-analysis}. For Sections~\ref{subsection:algorithm}, \ref{subsection:property-quotient}, \ref{subsection:structural-property}, and \ref{subsection:ratio-analysis}, we assume that $r\geq 2$ and $k^*\geq 120\log^2 r$. We discuss how to relax the assumption in Section~\ref{subsection:mixed-algorithm} in which we combine the designed algorithm with algorithms for other cases to obtain an algorithm with competitive ratio $O(\log^2 r)$. 
We will modify the algorithm in Section~\ref{section:poly-algorithm} to design an $O(\log^2 r)$-competitive algorithm that runs in polynomial time in each timestep, thereby completing the proof of Theorem~\ref{main-result:polymatroid}.

\subsection{Algorithm Description}\label{subsection:algorithm}
We assume that $k^*\geq 120\log^2 r$ and $r\geq 2$. The algorithm proceeds as follows: %When the element $e_t$ arrives, 
At each timestep $t\in [n]$, 
the algorithm computes $$q_t:=\min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}.$$ We note that $\mathcal{N}_t$ is a quotient of $f_{|\mathcal{N}_t}$ with $e_t\in \mathcal{N}_t$ and hence, $q_t$ is well-defined. Let $\ell_t:=\lceil \log q_t\rceil$. Then, the algorithm samples a value $R_t$ from $[\ell_t-3\lceil\log r\rceil, \ell_t+3\lceil\log r\rceil]$ uniformly at random. Finally, the algorithm sets $C(e_t)$ to be an integer picked uniformly at random from $[\lfloor2^{R_t}/(60\cdot \log ^2 r)\rfloor]$. We give a pseudocode of the algorithm in Algorithm~\ref{algo:pseudocode-polymatroid}.

\begin{algorithm2e}[ht]
\caption{Randomized Online Algorithm for \DPB}
\label{algo:pseudocode-polymatroid}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\LinesNumbered

\DontPrintSemicolon
  
    \KwInput{an ordering $e_1, e_2, \ldots, e_n$ of the ground set $\calN$ where $e_t$ is the element that arrives at time $t$ for each $t\in [n]$; $r=f(\mathcal{N})$, and 
    evaluation oracle access to $f_{|\calN_t}$ at each timestep $t\in [n]$, where  $f:2^{\calN}\rightarrow \Z_{\ge 0}$ is a polymatroid. 
    %a polymatroid $f:2^{\mathcal{N}}\rightarrow \mathbb{Z}_{\geq 0}$;
    %$r=f(\mathcal{N})$.
    }
    \KwOutput{color assignment $C: \mathcal{N} \rightarrow \mathbb{Z}_+$.}
    
    % Write Function with word ``Function''
    \SetKwProg{When}{When}{:}{}
    %\When{element $e_t$ arrives \ }{
    \For{$t=1, 2, \ldots, n$:}{
        $q_t\gets \min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}$
        
        $\ell_t\gets \lceil \log q_t \rceil$
        
        Sample $R_t$ $\textit{u.a.r.}$ from $[\ell_t-3\lceil\log r\rceil, \ell_t+3\lceil\log r\rceil]$

        Sample $C(e_t)$ $\textit{u.a.r.}$ from $[\lfloor2^{R_t}/(60\cdot \log ^2 r)\rfloor]$

        %\Return $C(e_t)$
    }
\end{algorithm2e}


\iffalse
\begin{algorithm2e}[h]
\caption{The Randomized Online Algorithm for Polymatroidal Disjoint Bases}
\label{algo:pseudocode-polymatroid}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\LinesNumbered

\DontPrintSemicolon
  
    \KwInput{elements of $\mathcal{N}$ arriving online;
    evaluation oracle access to a polymatroid $f:2^{\mathcal{N}}\rightarrow \mathbb{Z}_{\geq 0}$;
    $r=f(\mathcal{N})$.}
    \KwOutput{color assignment $C: \mathcal{N} \rightarrow \mathbb{Z}_+$.}
    
    % Write Function with word ``Function''
    \SetKwProg{When}{When}{:}{}
    \When{element $e_t$ arrives \ }{
        $q_t\gets \min \left\{|Q|: e_t\in Q \subseteq \mathcal{N}_t \ \& \ \text{$Q$ is a quotient of $f_{|\mathcal{N}_t}$}\right\}$
        
        $\ell_t\gets \lceil \log q_t \rceil$
        
        pick $r_t$ $\textit{u.a.r.}$ from $[\ell_t-3\lceil\log r\rceil, \ell_t+3\lceil\log r\rceil]$

        color element $e_t$ with color $C(e_t)$ picked $\textit{u.a.r.}$ from $[\lfloor2^{r_t}/(60\cdot \log ^2 r)\rfloor]$

        \Return $C(e_t)$
    }
\end{algorithm2e}
\fi

\subsection{Ordered Min-sized Quotients Property}\label{subsection:property-quotient}
%\znote{To Do: rename the section.}

In this section, we show %a structural property of $q_t$. 
%We recall that $q_t=\min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}$. 
%We prove 
that there can be at most $r$ distinct arrival times $t$ with the same value of $q_t$.

\begin{lemma}\label{lemma:counting-quotient}
%\knote{do we need to assume that $f(e)>0$ for every $e\in \calN$ for this lemma? Is it used in the proof?} 
    Let $f: 2^{\calN}\rightarrow \Z_{\ge 0}$ be a polymatroid over the ground set $\calN$ with $f(e)>0$ for every $e\in \mathcal{N}$ and $f(\emptyset)=0$. Let $e_1, e_2, \ldots, e_n$ be an ordering of the ground set $\calN$. For every $t\in [n]$, we define
\[
q_t:=\min\left\{|Q|: e_t\in Q\subseteq \calN_t \text{ and $Q$ is a quotient of $f_{|\calN_t}$}\right\}. 
\]
Then, for every $j\in \Z_+$,
\[
|\left\{t\in [n]: q_t = j\right\}| \le r.
\]

\iffalse
    \knote{This lemma is crucial and seems interesting by itself. I would prefer to state it completely with all hypothesis.}
\knote{
Let $f: 2^{\calN}\rightarrow \Z_{\ge 0}$ be a polymatroid over the ground set $\calN$ and let $e_1, e_2, \ldots, e_n$ be an ordering of the ground set $\calN$. Let 
\[
q_t:=\min\left\{|Q|: e_t\in Q\subseteq \calN_t \ \& \ \text{$Q$ is a quotient of $f_{|\calN_t}$}\right\} \ \forall t\in [n]. 
\]
Then, 
\[
|\left\{t\in [n]: q_t = j\right\}| \le r\ \forall\ j\in [n].
\]
}
\fi

\end{lemma}
\begin{proof}
    We note that $q_t$ is well-defined: empty set is closed since $f(e)>0$ for every $e\in \calN$ and hence, $\calN_t$ is a quotient of $f_{|\calN_t}$ containing $e_t$ for every $t\in [n]$. 
    Let $j\in \Z_+$. 
    Let $t_1<t_2<\ldots< t_{\ell}$ be the timesteps $t$ with $q_t=j$. It suffices to show that $\ell\leq r$. For every $i\in [\ell]$, let $Q_{t_i}$ be a minimum sized quotient of $f_{|\mathcal{N}_{t_i}}$ containing element $e_{t_i}$. We note that $|Q_{t_i}|=q_{t_i}=j$ for every $i\in [\ell]$. We define $S:=\bigcup_{i=1}^{\ell}\left(Q_{t_i}\setminus e_{t_i}\right)$.
    %\cnote{Shouldn't it say "let $Q_{t_i}$ be a min-sized quotient"?}

\iffalse
    \knote{
    Let $j\in \Z_+$. 
    Let $t_1<t_2<\ldots< t_{\ell}$ be the timesteps $t$ with $q_t=j$. It suffices to show that $\ell\leq r$. For every $i\in [\ell]$, let $Q_{t_i}$ be a quotient of $f_{|\mathcal{N}_{t_i}}$ containing element $e_{t_i}$ with $|Q_{t_i}|=q_{t_i}=j$ and $S_{t_i}:=Q_{t_i}\setminus e_{t_i}$. 
    
    We first show that $e_{t_a}\not\in S_{t_b}$ for every $a, b\in [\ell]$ with $a<b$. For the sake of contradiction, suppose there exist $a, b\in [\ell]$ with $a<b$ such that $e_{t_a}\in S_{t_b}$. By Lemma \ref{lemma:restrict-quotient}, $Q_{t_b}\cap \calN_{t_a}$ is a quotient of $f_{|\calN_{t_a}}$. We note that $|Q_{t_b}\cap \calN_{t_a}|<|Q_{t_b}|=j$ since $e_{t_b}\in Q_{t_{b}}$ and $e_{t_b}\not\in Q_{t_b}\cap \calN_{t_a}$. Consequently, $Q_{t_b}\cap \calN_{t_a}$ contradicts the fact that the smallest quotient of $f_{|\calN_{t_a}}$ containing element $e_{t_{a}}$ has size exactly $j$. Hence, $e_{t_a}\not\in S_{t_b}$ for every $a, b\in [\ell]$ with $a<b$. 

    Next, we show that $f(\calN_{t_i}\setminus S_{t_i})<f(\calN_{t_{i+1}}\setminus S_{t_{i+1}})$ for every $i\in [\ell-1]$. Let $i\in [\ell-1]$. Since $Q_{t_{i+1}}$ is a quotient of $\calN_{t_{i}+1}$ containing element $e_{t_{i}+1}$, we have that $f_{\mathcal{N}_{t_{i+1}}\setminus Q_{t_{i+1}}}(e_{t_{i+1}})>0$. We note that $\calN_{t_{i+1}-1}\setminus S_{t_{i+1}}=\calN_{t_{i+1}}\setminus Q_{t_{i+1}}$. Consequently, 
    $$f(\mathcal{N}_{t_{i+1}}\setminus S_{t_{i+1}})-f(\mathcal{N}_{t_{i+1}-1}\setminus S_{t_{i+1}}) 
    = f_{\mathcal{N}_{t_{i+1}-1}\setminus S_{t_{i+1}}}(e_{t_{i+1}}) 
    = f_{\mathcal{N}_{t_{i+1}}\setminus Q_{t_{i+1}}}(e_{t_{i+1}})
    >0,$$
    and hence $f(\calN_{t_{i+1}}\setminus S_{t_{i+1}})>f(\calN_{t_{i+1}-1}\setminus S_{t_{i+1}})$. Using this inequality with montonicity of the function $f$ implies that 
    \[
    f(\calN_{t_i}\setminus S_{t_i})\le f(\calN_{t_{i+1}-1}
    \]
    }
\fi

    We first show that $e_{t_i}\not\in S$ for every $i\in [\ell]$. Suppose there exists an element $e_{t_{i_1}}\in S$. Then, there exists an index $i_2\in [\ell]$ such that $e_{t_{i_1}}\in Q_{t_{i_2}}\setminus e_{t_{i_2}}$. Hence, $e_{t_{i_1}}\in Q_{t_{i_2}}\setminus e_{t_{i_2}} \subseteq \mathcal{N}_{t_{i_2}}$, which implies that $i_1\leq i_2$. Since $e_{t_{i_1}}\not\in Q_{t_{i_1}}\setminus e_{t_{i_1}}$, we have $i_1 \neq i_2$, which shows that $i_1<i_2$. By Lemma~\ref{lemma:restrict-quotient}, $Q_{t_{i_2}}\cap \mathcal{N}_{t_{i_1}}$ is a quotient of $f_{|\mathcal{N}_{t_{i_1}}}$. We note that $|Q_{t_{i_2}}\cap \mathcal{N}_{t_{i_1}}|<|Q_{t_{i_2}}|=j$ since $e_{t_{i_2}}\in Q_{t_{i_2}}$ and $e_{t_{i_2}}\not\in Q_{t_{i_2}}\cap \mathcal{N}_{t_{i_1}}$. Consequently, $Q_{t_{i_2}}\cap \mathcal{N}_{t_{i_1}}$ contradicts the fact that the smallest quotient of $f_{|\mathcal{N}_{t_{i_1}}}$ containing element $e_{t_{i_1}}$ has size exactly $j$. Hence, $e_{t_i}\not\in S$ for every $i\in [\ell]$.

    We now show that $f(\mathcal{N}_{t_i}\setminus S)<f(\mathcal{N}_{t_{i+1}}\setminus S)$ for every $i\in [\ell-1]$. Let $i\in [\ell-1]$. Since $Q_{t_{i+1}}$ is a quotient of $\mathcal{N}_{t_{i+1}}$ containing element $e_{t_{i+1}}$, we have $f_{\mathcal{N}_{t_{i+1}}\setminus Q_{t_{i+1}}}(e_{t_{i+1}})>0$. Since function $f$ is submodular, we have
    $$f(\mathcal{N}_{t_{i+1}}\setminus S)-f(\mathcal{N}_{t_{i+1}-1}\setminus S) = f_{\mathcal{N}_{t_{i+1}-1}\setminus S}(e_{t_{i+1}}) \geq f_{\mathcal{N}_{t_{i+1}}\setminus Q_{t_{i+1}}}(e_{t_{i+1}})>0.$$
    Hence,
    $$f(\mathcal{N}_{t_i}\setminus S)\leq f(\mathcal{N}_{t_{i+1}-1}\setminus S)<f(\mathcal{N}_{t_{i+1}}\setminus S),$$
    where the first inequality is by monotonicity of the function $f$. Thus, we have $f(\mathcal{N}_{t_i}\setminus S)<f(\mathcal{N}_{t_{i+1}}\setminus S)$ for every $i\in [\ell-1]$.

    This implies that $\{f(\mathcal{N}_{t_i}\setminus S)\}_{i=1}^{\ell}$ is a strictly increasing integer sequence. We note that $f(\mathcal{N}_{t_\ell}\setminus S)\leq r$. Also, since $f$ is a monotone function, we have $f(\mathcal{N}_{t_1}\setminus S)\geq f(e_{t_1})>0$. Hence, $\ell\leq r$.
    
\end{proof}

\iffalse
\knote{
\begin{remark}
For better understanding, we interpret Lemma~\ref{lemma:counting-quotient} for some concrete polymatroids defined on graphs. Let $G=(V,E)$ be a connected graph with $n=|V|$ vertices and $m=|E|$ edges.
\begin{enumerate}
    \item Lemma~\ref{lemma:counting-quotient} implies that for an arbitrary ordering of the edges $e_1, e_2, \ldots, e_m$ of $G$, there are at most $n-1$ distinct timesteps $t\in [m]$ with minimum $u_t-v_t$ cut in the graph $(V, E_t)$ being exactly $j$ for every $j\in Z_+$, where $E_t:=\{e_1, e_2, \ldots, e_t\}$ and $u_t, v_t$ are the end vertices of $e_t$. This follows by applying the lemma to the rank function $f: 2^E\rightarrow \Z_{\ge 0}$ of the graphic matroid defined by $G$. We recall that quotients of $f$ correspond to union of cut-sets and hence, $q_t$ is the minimum $u_t-v_t$ cut value in the graph $(V, E_t)$. 
    \item Lemma~\ref{lemma:counting-quotient} implies that for an arbitrary ordering of the edges $e_1, e_2, \ldots, e_m$ of $G$, there are at most $m-n+1$ distinct timesteps $t\in [m]$ at which the shortest cycle containing $e_t$ in the graph $(V, E_t)$ has length exactly $j$ for every $j\in Z_+$, where $E_t:=\{e_1, e_2, \ldots, e_t\}$. This follows by applying the lemma to the rank function $f: 2^E\rightarrow \Z_{\ge 0}$ of the cographic matroid defined by $G$. We recall that quotients of $f$ correspond to union of cycles and hence, $q_t$ is the length of the shortest cycle containing $e_t$ in the graph $(V, E_t)$. 
\end{enumerate}
\end{remark}
}
\fi

\begin{remark}
    For better understanding, we interpret Lemma~\ref{lemma:counting-quotient} for some concrete polymatroids defined on graphs. Let $G=(V,E)$ be a connected graph with $n=|V|$ vertices and $m=|E|$ edges. Let $e_1, e_2, \ldots, e_m$ be an arbitrary ordering of the edges in $E$. For every timestep $t\in [m]$, we define $E_t:=\{e_1, e_2, \ldots, e_t\}$.
    \begin{enumerate}
        \item Lemma~\ref{lemma:counting-quotient} implies that there are at most $n-1$ distinct timesteps $t\in [m]$ with minimum $u_t-v_t$ cut value in the graph $(V, E_t)$ being exactly $j$ for every $j\in Z_+$, where $u_t, v_t$ are the end vertices of $e_t$. This follows by applying the lemma to the rank function $f: 2^E\rightarrow \Z_{\ge 0}$ of the graphic matroid defined by $G$. We recall that quotients of $f$ correspond to union of cut-set of disjoint subsets of vertices, i.e., each quotient $Q\subseteq E$ is of the form $Q=\cup_{S\in \mathcal{C}}\delta(S)$, where $\mathcal{C}\subseteq 2^V\setminus \{\emptyset, V\}$ is a disjoint family. Hence, $q_t$ is the minimum $u_t-v_t$ cut value in the graph $(V, E_t)$.
        
        \item Lemma~\ref{lemma:counting-quotient} implies that there are at most $m-n+1$ distinct timesteps $t\in [m]$ at which the shortest cycle containing $e_t$ in the graph $(V, E_t)$ has length exactly $j$ for every $j\in Z_+$. This follows by applying the lemma to the rank function $f: 2^E\rightarrow \Z_{\ge 0}$ of the cographic matroid defined by $G$. We recall that quotients of $f$ correspond to union of cycles, i.e., each quotient $Q\subseteq E$ is of the form $Q=\cup_{F\subseteq \mathcal{F}}F$, where $\mathcal{F}$ is a collection of cycles in $G$. Hence, $q_t$ is the length of the shortest cycle containing $e_t$ in the graph $(V, E_t)$. 
    \end{enumerate}
\end{remark}

\iffalse
\paragraph{Remark.} For better understanding, we interpret Lemma~\ref{lemma:counting-quotient} for some special polymatroids defined on graphs. Let $G=(V,E)$ be a connected graph with $n=|V|$ vertices and $m=|E|$ edges. Let $e_1, e_2, \ldots, e_m$ be an arbitrary arrival order of $E$, where $e_t$ arrives at time $t$ for every $t\in [m]$. We define $E_t:=\{e_i\in E: i\in [t]\}$ be the set of edges that have arrived until time $t$ for every $t\in [m]$.

\begin{enumerate}
    \item Suppose $f$ is the rank function of the graphic matroid defined by $G$. We have $f(A)=|V|-c(V,A)$ for every $A\subseteq E$, where $c(V,A)$ is the number of components in the graph $(V,A)$. The function value on the ground set equals $r=f(E)=|V|-1=n-1$. We note that a quotient $Q\subseteq E$ is a cut in graph $G$ \knote{We note that quotients correspond to union of cut-sets in the graph, i.e., each quotient $Q\subseteq E$ is of the form $Q=\cup_{S\in \mathcal{C}}\delta(S)$, where $\mathcal{C}\subseteq 2^V\setminus \{\emptyset, V\}$.}. Hence, for every $t\in [m]$, the value $q_t$ is equal to the minimum $u_t-v_t$ cut value in the graph $(V,E_t)$, where $u_t$ and $v_t$ are the two endpoints of edge $e_t$. Lemma~\ref{lemma:counting-quotient} implies that for every $j\in \mathbb{Z}_+$, there are at most $n-1$ distinct timesteps $t\in [m]$ with minimum $u_t-v_t$ cut in the graph $(V, E_t)$ being exactly $j$.

    

    \item Suppose $f$ is the rank function of the cographic matroid defined by $G$. We have $f(A)=|A|+1-c(V,E\setminus A)$ for every $A\subseteq E$, where $c(V,A)$ is the number of components in the graph $(V,A)$. The function value on the ground set equals $r=f(E)=|E|+1-|V|=m-n+1$. Since we assumed that $f({e})>0$ for every edge $e\in E$, this implies that graph $G$ is a union of cycles \knote{why is this relevant? Also, it implies that $c(V, E-e)\le 1$ for every $e\in E$ which is equivalent to saying that the graph has no bridge, i.e., no cut edge which is equivalent to saying that the graph is $2$-edge-connected. I don't see why it implies that $G$ is a union of cycles.}. For a quotient $Q\subseteq E$, we have $f(E\setminus Q)<f(E\setminus Q+e)$ for every $e\in Q$, which implies that $c(V,Q)+1>c(V,Q-e)$. This implies that $Q$ is a union of cycles.\knote{Shorten the previous two sentences to simply say: We note that quotients of $f$ correspond to union of cycles in the graph, i.e., each quotient $Q\subseteq E$ is of the form $Q=\cup_{F\subseteq \mathcal{F}}F$, where $\mathcal{F}$ is a collection of cycles in $G$.} Hence, for every $t\in [m]$, the value $q_t$ is equal to the minimum cycle containing edge $e_t$ \knote{in the graph $(V, E_t)$?}. Lemma~\ref{lemma:counting-quotient} implies that for every $j\in \mathbb{Z}_+$, there are at most $m-n+1$ distinct timesteps $t\in [m]$ with minimum cycle containing $e_t$ in graph $(V,E_t)$ being exactly $j$.
\end{enumerate}
\fi

%\knote{Interpret Lemma \ref{lemma:counting-quotient} for the graphic/cographic matroid rank function. Might be worth discussing its meaning for graphs. Can we use this lemma to provide a new proof that the number of min-cuts is polynomial (maybe not $O(n^2)$ but some polynomial)?} 

%\znote{I haven't figured out how to bound the number of global min-cuts. We have some information on the number of timesteps with current min-cut being some fixed value. But there might be multiple different min-cuts correspond to the same timestep.}
%\knote{I think for the cographic matroid rank, $q_t$ is the size of the smallest cycle containing the element; if we just have $2$ vertices and all edges are simply parallel edges between these two vertices, then wouldn't $q_t=2$ for all edges and for all timesteps? Yes, but this doesn't contradict the lemma.}

\subsection{Structural Property}\label{subsection:structural-property}
For each $t \in [n]$, we define the element $e_t$ to be \emph{good} if $\frac{k^*}{2r}< q_t < 2rk^*$ and \emph{bad} otherwise. Let $\mathcal{N}_{\good}$ be the set of good elements. 
%Let $g:2^{\calN_{\good}}$ be the function defined as $g:=f_{|\calN_{\good}}$.
We define the following counterpart of $k^*$. 
\begin{equation}
    k^*_{\text{onl}}:=\min_{A\subseteq \mathcal{N}_{\good}: f(A)<f(\mathcal{N}_{\good})} \frac{\sum_{e\in \mathcal{N}_{\good}}f_A(e)}{f(\mathcal{N}_{\good})-f(A)}. \label{def:new-opt-k}
\end{equation}
The following is the main result of this section. It shows that bases of $f_{|\calN_{\good}}$ are also bases of $f$ and moreover, the quantity $k^*_{\text{onl}}$ that depends on the set of good elements is at least a constant fraction of $k^*$. 
\begin{restatable}{lemma}{lemmaGoodOpt}\label{lemma:new-opt}
We have that 
\begin{enumerate}
    \item $f(\calN_{\good})=f(\calN)$ and 
    \item $k_{\text{onl}}^*\ge \frac{1}{2} k^*$. 
\end{enumerate}
\end{restatable}
We prove Lemma \ref{lemma:new-opt} in a series of steps. 
We note that an element $e_t$ could be bad because of two reasons: either $q_t$ is too large or too small. 
We first show that the only reason for certain elements being bad is that their $q_t$ is too small. 
%The following lemma shows that dropping all bad elements will not decrease the value of $k^*$ by more than a constant factor.

\begin{lemma}\label{lemma:q_t-upper-bound}
    Let $A\subseteq \mathcal{N}$ be a closed set of $f$. Let $T\geq 1$ be the smallest integer such that
    \begin{equation}\label{inequality-for-bad:k^*}
    \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{equation}
    Then, for every element $e_t\in \mathcal{N}_T\setminus A$ with $t\in [T]$, we have that $q_t<2rk^*$. 
\end{lemma}
\begin{proof}
%We note that $T$ is well-defined since $\sum_{e\in \calN_t\setminus A}(f(A+e)-f(A))$ is non-decreasing with $t$. 
    By definition of $k^*$, we have
    $$
    \sum_{e\in \mathcal{N}\setminus A} \left(f(A+e)-f(A)\right) \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    $$
    Since $T$ is the smallest integer satisfying inequality~(\ref{inequality-for-bad:k^*}), we have
    \begin{equation}\label{inequality:new-T}
        \sum_{e\in \mathcal{N}_{T-1}\setminus A} \left(f(A+e)-f(A)\right) < k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{equation}
    Hence,
    \begin{align}\label{inequality:contribution-upper-bound}
        \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) &= \left(\sum_{e\in \mathcal{N}_{T-1}\setminus A} \left(f(A+e)-f(A)\right)\right)+\left(f(A+e_{T})-f(A)\right) \notag \\
        &< k^*\cdot \left(f(\mathcal{N})-f(A)\right)+\left(f(A+e_{T})-f(A)\right) \ \ \text{(by inequality~(\ref{inequality:new-T}))} \notag \\
        &\leq k^*\cdot \left(f(\mathcal{N})-f(A)\right)+\left(f(\mathcal{N})-f(A)\right) \ \ \text{(since $f(A+e_T)\leq f(\mathcal{N})$)} \notag \\
        &= (k^*+1)\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{align}
    Since $A$ is a closed set, we have $f(A+e)-f(A)\geq 1$ for every element $e\in \mathcal{N}_T\setminus A$. Thus, using inequality~(\ref{inequality:contribution-upper-bound}), we have
    \begin{equation}\label{inequality:size-upper-bound}
        |\mathcal{N}_T\setminus A| < \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) \leq (k^*+1)\cdot (f(\mathcal{N})-f(A)) \leq (k^*+1)r <2rk^*.
    \end{equation}
    
    Since $A$ is a closed set, $\mathcal{N}\setminus A$ is a quotient of $f$. By Lemma~\ref{lemma:restrict-quotient}, for every $t\in [n]$, we know that $\mathcal{N}_t\setminus A$ is a quotient of $f_{|\mathcal{N}_t}$. Hence, for every element $e_t\in \mathcal{N}_T\setminus A$ with $t\in [T]$, we have that $q_t\leq |\mathcal{N}_t\setminus A|\leq |\mathcal{N}_T\setminus A|<2rk^*$, where the last inequality is by inequality~(\ref{inequality:size-upper-bound}).
\end{proof}

Next, we show that dropping all bad elements will not decrease the value of $k^*$ by more than a constant factor for closed sets. We first show this for closed sets (Lemma \ref{lemma:new-ratio-closed}) and derive it for arbitrary sets as a corollary (Corollary \ref{corollary:new-ratio}). 
\begin{lemma}\label{lemma:new-ratio-closed}
    For every closed set $A\subseteq \mathcal{N}$,
    $$\sum_{e\in \mathcal{N}_{\good}\setminus A} \left(f(A+e)-f(A)\right) \geq \frac{k^*}{2}\cdot \left(f(\mathcal{N})-f(A)\right).$$
\end{lemma}
\begin{proof}
Let $A\subseteq \mathcal{N}$ be a closed set. 
%We note that $\sum_{e\in \calN_t\setminus A}(f(A+e)-f(A))$ is non-decreasing with $t$. 
Let $T\geq 1$ be the smallest integer such that inequality \eqref{inequality-for-bad:k^*} holds. 
    \iffalse
    Let $A\subseteq \mathcal{N}$ be a closed set. By definition of $k^*$, we have
    $$
    \sum_{e\in \mathcal{N}\setminus A} \left(f(A+e)-f(A)\right) \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    $$
    Let $T\geq 1$ be the smallest integer satisfying  
    \begin{equation}\label{inequality:k^*}
    \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{equation}
    Since $T$ is the smallest integer satisfying inequality~(\ref{inequality:k^*}), we have
    \begin{equation}\label{inequality:new-T}
        \sum_{e\in \mathcal{N}_{T-1}\setminus A} \left(f(A+e)-f(A)\right) < k^*\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{equation}
    Hence,
    \begin{align}\label{inequality:contribution-upper-bound}
        \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) &= \left(\sum_{e\in \mathcal{N}_{T-1}\setminus A} \left(f(A+e)-f(A)\right)\right)+\left(f(A+e_{T})-f(A)\right) \notag \\
        &< k^*\cdot \left(f(\mathcal{N})-f(A)\right)+\left(f(A+e_{T})-f(A)\right) \ \ \text{(by inequality~(\ref{inequality:new-T}))} \notag \\
        &\leq k^*\cdot \left(f(\mathcal{N})-f(A)\right)+\left(f(\mathcal{N})-f(A)\right) \ \ \text{(since $f(A+e_T)\leq f(\mathcal{N})$)} \notag \\
        &= (k^*+1)\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{align}
    Since $A$ is a closed set, we have $f(A+e)-f(A)\geq 1$ for every element $e\in \mathcal{N}_T\setminus A$. Thus, using inequality~(\ref{inequality:contribution-upper-bound}), we have
    \begin{equation}\label{inequality:size-upper-bound}
        |\mathcal{N}_T\setminus A| < \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) \leq (k^*+1)\cdot (f(\mathcal{N})-f(A)) \leq (k^*+1)r <2rk^*.
    \end{equation}
    
    Since $A$ is a closed set, $\mathcal{N}\setminus A$ is a quotient of $f$. By Lemma~\ref{lemma:restrict-quotient}, for every $t\in [n]$, we know that $\mathcal{N}_t\setminus A$ is a quotient of $f_{|\mathcal{N}_t}$. Hence, for every element $e_t\in \mathcal{N}_T\setminus A$ with $t\in [T]$, $q_t\leq |\mathcal{N}_t\setminus A|\leq |\mathcal{N}_T\setminus A|<2rk^*$, where the last inequality is by inequality~(\ref{inequality:size-upper-bound}). This implies that for every $t\in [T]$, element $e_t\in \mathcal{N}_T\setminus A$ is bad if and only if $q_t\leq \frac{k^*}{2r}$. Hence, we have

    \fi
    Lemma \ref{lemma:q_t-upper-bound} implies that for every $t\in [T]$, element $e_t\in \mathcal{N}_T\setminus A$ is bad if and only if $q_t\leq \frac{k^*}{2r}$. Hence, we have
    \begin{align}\label{inequality:good-elements}
        |\mathcal{N}_T \setminus (A\cup \mathcal{N}_{\good})| &= |\{t\in [T]: e_t\in \mathcal{N}_T\setminus (A\cup \mathcal{N}_{\good})\}| = \left|\left\{t\in [T] : e_t\in\mathcal{N}_T\setminus A \ \& \ q_t\leq \frac{k^*}{2r} \right\}\right| \notag \\
        &\leq \left|\left\{t\in [T] : q_t\leq \frac{k^*}{2r} \right\}\right| = \sum_{j=1}^{\lfloor \frac{k^*}{2r}\rfloor} \left|\{t\in [T] : q_t=j\}\right| \notag \\
        &\leq \left(\frac{k^*}{2r}\right) r \ \ \text{(by Lemma~\ref{lemma:counting-quotient})} \notag \\
        &= \frac{k^*}{2}.
    \end{align}
    
    Thus,
    $$\begin{aligned}
        &\sum_{e\in \mathcal{N}_{\good}\setminus A} \left(f(A+e)-f(A)\right) \\
        &\quad \quad \quad \geq \sum_{e\in (\mathcal{N}_T \cap\mathcal{N}_{\good})\setminus A} \left(f(A+e)-f(A)\right) \ \ \text{(since $f(A+e)\geq f(A)$ for every $e\in \mathcal{N}$)}\\
        &\quad \quad \quad = \sum_{e\in \mathcal{N}_T\setminus A} \left(f(A+e)-f(A)\right) - \sum_{e\in \mathcal{N}_T \setminus (A\cup \mathcal{N}_{\good})} \left(f(A+e)-f(A)\right)\\
        &\quad \quad \quad \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right) - \sum_{e\in \mathcal{N}_T \setminus (A\cup \mathcal{N}_{\good})} \left(f(A+e)-f(A)\right) \ \ \text{(by inequality~(\ref{inequality-for-bad:k^*}))}\\
        &\quad \quad \quad \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right) - \sum_{e\in \mathcal{N}_T \setminus (A\cup \mathcal{N}_{\good})} \left(f(\mathcal{N})-f(A)\right) \ \ \text{(by monotonicity of $f$)}\\
        &\quad \quad \quad \geq k^*\cdot \left(f(\mathcal{N})-f(A)\right) - \frac{k^*}{2}\cdot \left(f(\mathcal{N})-f(A)\right) \ \ \text{(by inequality~(\ref{inequality:good-elements}))}\\
        &\quad \quad \quad = \frac{k^*}{2}\cdot \left(f(\mathcal{N})-f(A)\right).
    \end{aligned}$$
\end{proof}

\begin{corollary}\label{corollary:new-ratio}
    For every set $A\subseteq \mathcal{N}$,
    $$\sum_{e\in \mathcal{N}_{\good}\setminus A} \left(f(A+e)-f(A)\right) \geq \frac{k^*}{2}\cdot \left(f(\mathcal{N})-f(A)\right).$$
\end{corollary}
\begin{proof}
    We have
    $$\begin{aligned}
        \sum_{e\in \mathcal{N}_{\good}\setminus A} (f(A+e)-f(A)) &\geq \sum_{e\in \mathcal{N}_{\good}\setminus \text{span}(A)} (f(A+e)-f(A)) \ \ \text{(since $A\subseteq \text{span}(A)$)}\\
        &\geq \sum_{e\in \mathcal{N}_{\good}\setminus \text{span}(A)} (f(\text{span}(A)+e)-f(\text{span}(A)) \\ 
        & \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{(since $f_A(e)\geq f_{\text{span}(A)}(e)$ by submodularity of $f$)} \\
        &\geq \frac{k^*}{2} \cdot (f(\mathcal{N})-f(\text{span}(A))) \ \ \text{(by applying Lemma~\ref{lemma:new-ratio-closed} for $\text{span}(A)$)}\\
        &= \frac{k^*}{2}\cdot (f(\mathcal{N})-f(A)). \ \ \text{(since $f(A)=f(\text{span}(A))$)}
    \end{aligned}$$
\end{proof}

We now restate and prove the main lemma of this section.
\lemmaGoodOpt*
\iffalse
Let $k^*_{\text{onl}}$ be the corresponding upper bound for the optimum with respect to good elements, i.e.,
\begin{equation}
    k^*_{\text{onl}}:=\min_{A\subseteq \mathcal{N}_{\good}: f(A)<f(\mathcal{N}_{\good})} \frac{\sum_{e\in \mathcal{N}_{\good}}f_A(e)}{f(\mathcal{N}_{\good})-f(A)}. \label{def:new-opt-k}
\end{equation}
The following corollary shows that $k^*_{\text{onl}}$ is at least half of $k^*$.

\begin{corollary}\label{corollary:new-opt}
    $k_{\text{onl}}^*\geq \frac{1}{2}k^*$.
\end{corollary}
\fi
\begin{proof}
%\knote{There are still several $\calN_{\text{onl}}$ in Section 3 which need to be replaced by $\calN_{\good}$. Proofread and replace carefully.}
    By applying Corollary~\ref{corollary:new-ratio} for $A=\mathcal{N}_{\good}$, we conclude that $f(\mathcal{N})=f(\mathcal{N}_{\good})$ since $k^*>0$ by assumption. Hence,
    $$k^*_{\text{onl}}=\min_{A\subseteq \mathcal{N}_{\good}: f(A)<f(\mathcal{N}_{\good})} \frac{\sum_{e\in \mathcal{N}_{\good}}f_A(e)}{f(\mathcal{N})-f(A)}=\min_{A\subseteq \mathcal{N}_{\good}: f(A)<f(\mathcal{N}_{\good})} \frac{\sum_{e\in \mathcal{N}_{\good}\setminus A}f_A(e)}{f(\mathcal{N})-f(A)},$$
    where the last equality holds since $f_A(e)=0$ for every $e\in A$. By Corollary~\ref{corollary:new-ratio}, for every set $A\subseteq \mathcal{N}$, we have
    $$\frac{\sum_{e\in \mathcal{N}_{\good}\setminus A}f_A(e)}{f(\mathcal{N})-f(A)}\geq \frac{k^*}{2}.$$
    Hence, $k_{\text{onl}}^*\geq \frac{1}{2}k^*$.
\end{proof}

\subsection{Competitive Ratio Analysis}\label{subsection:ratio-analysis}
Now, we analyze the competitive ratio of Algorithm~\ref{algo:pseudocode-polymatroid}. 
Let $h:=\lfloor \log k^* \rfloor$. We note that $\frac{k^*}{2}< 2^h \leq k^*$. We now prove that every color $c\in [\lfloor 2^h/ (60\cdot \log^2 r)\rfloor]$ is a base color with constant probability in Algorithm~\ref{algo:pseudocode-polymatroid}.

\begin{lemma}\label{lemma:polymatroid-proper-color-probability}
    Let $c \in [\lfloor 2^h/ (60\cdot \log^2 r)\rfloor]$. Then, $\mathbf{Pr}_{\texttt{Alg$_1$} }[c \text{ is a base color}]\geq \frac{1}{2}$.
\end{lemma}
\begin{proof}
    By Lemma \ref{lemma:new-opt}, we have that $f(\calN_{\good})=f(\calN)$ and hence, bases of $f|_{\calN_{\good}}$ correspond to bases of $f$. By Lemma \ref{lemma:new-opt}, we also have that  
    $k_{\text{onl}}^*\geq \frac{k^*}{2}\geq 2^{h-1}$. Let $e_t\in \mathcal{N}_{\good}$. We have $\frac{k^*}{2r}< q_t < 2rk^*$ and hence, $\lceil \log q_t \rceil -3\lceil \log r\rceil \leq h\leq \lceil \log q_t \rceil+3\lceil \log r \rceil$. Therefore,
    \begin{equation}\label{inequality:probability-analysis}
        \mathbf{Pr}[R_t=h]=\frac{1}{6\lceil \log r \rceil+1}>\frac{1}{15\log r}.
    \end{equation}
    Hence, for every element $e_t\in \mathcal{N}_{\good}$, the probability that $e_t$ is colored with $c$ is
    $$\begin{aligned}
        \mathbf{Pr}[C(e_t)=c] &\geq \mathbf{Pr}[R_t=h]\cdot \mathbf{Pr}[C(e_t)=c|r_t=h] \\
        &= \mathbf{Pr}[R_t=h] \cdot \frac{1}{\lfloor 2^h/ (60\cdot \log^2 r)\rfloor} \\
        &> \frac{1}{15\log r}\cdot \frac{60\cdot \log^2 r}{2^h} \ \ \text{(by inequality~(\ref{inequality:probability-analysis}))}\\
        &\geq \frac{1}{15\log r}\cdot \frac{60\cdot \log^2 r}{2k_{\text{onl}}^*}= \frac{2\log r}{k^*_{\text{onl}}}.
    \end{aligned}$$
    By applying Lemma~\ref{lemma:sampling-property} for the polymatroid $f_{|\mathcal{N}_{\good}}$, we conclude that the elements in $\mathcal{N}_{\good}$ with color $c$ form a base of $f_{|\mathcal{N}_{\good}}$ with probability at least $\frac{1}{2}$. We recall that bases of $f_{|\calN_{\good}}$ are also bases of $f$. 
    %By applying Corollary~\ref{corollary:new-ratio} for $A=\mathcal{N}_{\good}$, we conclude that $f(\mathcal{N})=f(\mathcal{N}_{\good})$ since $k^*\geq 2$. 
    Hence, $c$ is a base color with probability at least $\frac{1}{2}$.
\end{proof}

Lemma \ref{lemma:polymatroid-proper-color-probability} implies a lower bound on the expected number of base colors obtained by Algorithm~\ref{algo:pseudocode-polymatroid}.

\begin{corollary}\label{corollary:number-proper-colors}
    The expected number of base colors obtained by Algorithm~\ref{algo:pseudocode-polymatroid} is at least $$\mathbb{E}[\texttt{Alg$_1$}(f)]\geq \frac{1}{2}\cdot \lfloor 2^h/ (60\cdot \log^2 r)\rfloor.$$
\end{corollary}
\begin{proof}
%Let $\texttt{Alg$_1$}(f)$ denote the number of base colors obtained by Algorithm~\ref{algo:pseudocode-polymatroid}. 
By Lemma \ref{lemma:polymatroid-proper-color-probability}, we have that 
    $$\begin{aligned}
        \mathbb{E}[\texttt{Alg$_1$}(f)] &= \sum_{c\in [\lfloor 2^h/ (60\cdot \log^2 r)\rfloor]} \mathbf{Pr}_{\texttt{Alg$_1$} }[c \text{ is a base color}] 
        %&\geq \sum_{c\in [\lfloor 2^h/ (60\cdot \log^2 r)\rfloor]} \frac{1}{2} \ \ \text{(by Lemma~\ref{lemma:proper-color-probability})} \\
        &\ge \frac{1}{2}\cdot \lfloor 2^h/ (60\cdot \log^2 r)\rfloor.
    \end{aligned}$$
\end{proof}

%\knote{Would be good to write a remark to clarify where the assumptions that $r\ge 2$ and $k^*\ge \log^2{r}$ are used in the proof.}
%\znote{Added a remark after section 3.5, since the assumption $k^*>=120\log^2 r$ is used there.}

\subsection{Combined Algorithm}\label{subsection:mixed-algorithm}
We recall that our analysis of Algorithm~\ref{algo:pseudocode-polymatroid} assumed that $r\geq 2$ and $k^*\geq 120\log^2 r$. We now combine Algorithm~\ref{algo:pseudocode-polymatroid} with other algorithms to address all ranges of $r$ and $k^*$.

Consider the online algorithm \texttt{Alg$_1^*$} that runs Algorithm~\ref{algo:pseudocode-polymatroid} with probability $\frac{1}{3}$, assigns $C(e_t)=1$ for every element $e_t$ with probability $\frac{1}{3}$, and assigns $C(e_t)=t$ for every element $e_t$ with probability $\frac{1}{3}$. We now show that the resulting online algorithm \texttt{Alg$_1^*$} has competitive ratio $O(\log^2 r)$.

\begin{theorem}\label{theorem:polymatroid-combined-ratio}
    Algorithm \texttt{Alg$_1^*$} has competitive ratio $O(\log^2 r)$.
\end{theorem}
\begin{proof}
    Suppose $r=1$. Then, each singleton forms a base, which implies that $\opt(f)=n$. We recall that the algorithm assigns $C(e_t)=t$ for every element $e_t$ with probability $\frac{1}{3}$. This implies that
    $$\begin{aligned}
        \mathbb{E}[\texttt{Alg$_1^*$}(f)] \geq \frac{1}{3}\cdot \opt(f).
    \end{aligned}$$

    Suppose $r\geq 2$ and $k^*< 120\log^2 r$. Then, the optimum is also smaller than $120\log^2 r$ by Theorem~\ref{thm:CCV-k^*}. We recall that the algorithm assigns $C(e_t)=1$ for every element $e_t$ with probability $\frac{1}{3}$. This implies that
    $$\begin{aligned}
        \mathbb{E}[\texttt{Alg$_1^*$}(f)] \geq \frac{1}{3} > \frac{1}{360\log^2 r}\cdot \opt(f).
    \end{aligned}$$

    Now, we may assume that $k^*\geq 120\log^2 r$ and $r\geq 2$. We recall that the algorithm \texttt{Alg$_1^*$} runs Algorithm~\ref{algo:pseudocode-polymatroid} with probability $\frac{1}{3}$. We have
    \begin{equation}\label{inequality:positive-assumption-k}
    2^h/ (60\cdot \log^2 r)> \frac{1}{60}\cdot \frac{k^*}{2\log^2 r}\geq 1,
    \end{equation}
    which implies that
    \begin{equation}\label{inequality:trunc-integer}
        \lfloor 2^h/ (60\cdot \log^2 r) \rfloor \geq \frac{1}{2}\cdot 2^h/ (60\cdot \log^2 r).
    \end{equation}
    Hence, we have
    $$\begin{aligned}
        \mathbb{E}[\texttt{Alg$_1^*$}(f)]&\geq \frac{1}{3}\cdot \mathbb{E}[\texttt{Alg$_1$}(f)] \\
        &\geq \frac{1}{6}\cdot \lfloor 2^h/ (60\cdot \log^2 r)\rfloor \ \ \text{(by Corollary~\ref{corollary:number-proper-colors})}\\
        &\geq \frac{1}{12}\cdot 2^h/ (60\cdot \log^2 r) \ \ \text{(by inequality~(\ref{inequality:trunc-integer}))}\\
        &\geq \frac{1}{1440\cdot \log^2r}\cdot k^* \\
        &\geq \frac{1}{1440\cdot \log^2r}\cdot \opt(f). \ \ \text{(by Theorem~\ref{thm:CCV-k^*})}
    \end{aligned}$$
\end{proof}

\begin{remark}
    We recall that we assumed $k^*\geq 120\log^2 r$ and $r\geq 2$ in Sections~\ref{subsection:algorithm}, \ref{subsection:property-quotient}, \ref{subsection:structural-property}, and \ref{subsection:ratio-analysis}. The first assumption is to ensure the correctness of inequality~(\ref{inequality:positive-assumption-k}), which is used in the last case of the proof for Theorem~\ref{theorem:polymatroid-combined-ratio}. The second assumption is used for inequality~(\ref{inequality:probability-analysis}) in the proof for Lemma~\ref{lemma:polymatroid-proper-color-probability}.
\end{remark}

==> submodular-algorithm.tex <==
\section{Faster Algorithm for Hypergraph Matroids}\label{section:hypergraph-faster-algo}
\znote{To do...}

In this section, we show a more general result for general polymatroids. A polymatroid $f:2^\mathcal{N}\rightarrow \mathbb{Z}_+$ is a monotone submodular function with $f(\emptyset)=0$ and $f(\mathcal{N})=r$. We call $S\subseteq \mathcal{N}$ a \emph{base} if $f(S)=f(\mathcal{N})$. The input to the \emph{Disjoint Bases of Polymatroids} (DBP) problem is an oracle of $f$. The output is a color assignment $C:\mathcal{N}\rightarrow \mathbb{Z}_+$ which maximizes the number of proper colors $c\in \mathbb{Z}_+$, where color $c$ is called a \emph{proper color} if the elements with color $c$ forms a base. In the \emph{Online Disjoint Bases of Polymatroids} (Online-DBP) problem, $r=f(\mathcal{N})$ is known in advance while the elements $\mathcal{N}=\{e_1, \ldots, e_m\}$ come in an online fashion, where element $e_t$ arrives at time $t$ for every $1\leq t \leq m$. An Online-DBP algorithm has to decide on the color $C(e_t)$ once it arrives. We show that there exists a purely $O(\log^2 r)$-competitve randomized algorithm.

\begin{theorem}
    For the Disjoint Bases of Polymatroids problem, there exists a randomized online algorithm with pure competitive ratio $O(\log^2 r)$.
\end{theorem}

\subsection{Preliminaries.}
Let $f:2^\mathcal{N}\rightarrow \mathbb{Z}_+$ be an integer-valued set function over $\mathcal{N}$. $f$ is monotone if $f(S)\leq f(T)$ for every $S\subseteq T$. $f$ is submodular if $f(S)+f(T)\geq f(S\cup T)+f(S\cap T)$ for every $S, T\subseteq \mathcal{N}$. For every $S,T\subseteq \mathcal{N}$, define $f(S|T):=f(S\cup T)-f(T)$. Equivalently, $f$ is submodular if $f(S|T)$ if non-increasing in $T$ for every $S,T\subseteq \mathcal{N}$.

Let $f:2^\mathcal{N}\rightarrow \mathbb{Z}_+$ be a polymatroid. For a set $S\subseteq \mathcal{N}$, the span of $S$ is defined as the set of elements with marginal value $0$ with respect to $S$, i.e., $\text{span}(S):=\{e:f(e|S)=0\}$. We note that $\text{span}(S)$ is monotonically increasing. A set $S$ is called a \emph{closed set} if $S=\text{span}(S)$. A \emph{quotient} $Q$ of $f$ is defined as any set that is the complement of a closed set. Equivalently, $Q$ is a quotient iff $Q=\mathcal{N}\setminus \text{span}(S)$ for some set $S$.

==> techniques-1.tex <==
\subsection{Techniques}
%\knote{Define quotients, state the estimate, and highlight Lemma \ref{lemma:counting-quotient} as the novel structural property. Explain how the lemma is useful to design an online algorithm with polylog competitive ratio.}

Let us first consider \DSC, where the polymatroid $f$ is defined to be the coverage function of the input hypergraph $H=(V,E)$. We let $n:=|V|$ be the number of vertices and $m:=|E|$ be the number of hyperedges. As we have mentioned before, the quantity $k^*(f)$ equals the min-degree $\delta_H$ of $H$. If the min-degree $\delta_H$ is known in advance, Pananjady, Bagaria, and Vaze \cite{PBV15} showed that sampling the color of each hypergraph uniformly from the palette $[\Theta(\delta_H/\log n)]$ would lead to $\Omega(\delta_H/\log n)$ base colors. Emek, Goldbraikh, and Kantor \cite{EGK19} presented a randomized online algorithm without prior knowledge of $\delta_H$. Their algorithm works as follows: When hyperedge $e_t$ arrives, the algorithm first computes the min-degree $\delta_t$ of a vertex in $e_t$ in the hypergraph containing all hyperedges that have arrives so far. By a combinatorial lemma, they showed that $\delta_t\leq \delta_H\leq \delta_t\cdot O(n)$ for a constant fraction of timesteps $t\in [m]$. Their algorithm then 
%guesses the value of $\delta$ by sampling 
samples 
$P_t$ uniformly from $\{\delta_t\cdot 2^0, \delta_t\cdot 2^1, \delta_t\cdot 2^2, \ldots, \delta_t\cdot 2^{O(\log n)}\}$. We note that if $\delta_t\le \delta_H\le \delta_t\cdot O(n)$, then $P_t$ is a $2$-approximation of $\delta_H$ with probability $\Omega(\frac{1}{\log n})$. Finally, the algorithm samples the color $C(e_t)$ of the hyperedge $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 n)]$. Since expected $\Omega(1/\log n)$ fraction of timesteps obtain a $2$-approximation of $\delta_H$, the algorithm achieves $\Omega(\delta_H/\log ^2n)$ base colors in expectation. We note that $\opt(f)\le k^*(f) = \delta_H$ and hence the competitive ratio is $O(\log^2 n)$. 

In this work, our main contribution is appropriately generalizing the above ideas to \DPB. Let $r:=f(\mathcal{N})$ be the rank of the polymatroid $f$. For the discussion here, we will assume that $r\geq 2$ and $k^*(f)=\Omega(\log^2 r)$ since this is the non-trivial case. This assumption can be relaxed by combining the algorithm for this case with those designed for other cases, as detailed in Section~\ref{subsection:mixed-algorithm}. If we know $k^*(f)$ in advance, then sampling the color of each element uniformly from the palette $[\Theta(k^*(f)/\log r)]$ gives $\Omega(k^*(f)/\log{r})$ base colors. To prove this, we show that the subset obtained by picking each element in $\mathcal{N}$ with probability $\Omega(\log r/k^*(f))$ independently at random is a base of polymatroid $f$ with constant probability (see Lemma~\ref{lemma:sampling-property}). Hence, every color in the palette is a base color with constant probability, which implies $\Omega(k^*(f)/\log r)$ base colors.

Now, we are in the online model where $k^*(f)$ is not known in advance. To address this situation, we will \emph{estimate} $k^*(f)$ at each timestep. 
%Adapting the idea used in \DSC, our algorithm has the following framework: 
When element $e_t$ arrives, suppose that we can estimate $q_t$ of $k^*(f)$. At each timestep, If we can compute an estimate $q_t$ that is within a $\text{poly}(r)$ factor of $k^*(f)$, that is, $\Theta\left(\frac{k^*(f)}{\text{poly}(r)}\right)\leq q_t \leq \Theta(k^*(f)\cdot \text{poly}(r))$. Then, we can obtain a $2$-approximation $P_t$ of $k^*(f)$ with probability $\Omega(1/\log r)$ by sampling $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$. In this way, sampling the color $C(e_t)$ of the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$ would lead to $\Omega(k^*(f)/ \log^2 r)$ base colors on expectation.

Hence, the key challenge is to estimate $k^*(f)$ with only part of elements known. Although we do not know how to estimate $k^*(f)$ within a $\text{poly}(r)$ factor, we will achieve this for enough timesteps. For a timestep $t\in [n]$, we call it a \emph{good} timestep if our estimate $q_t$ is within a $\text{poly}(r)$ factor of $k^*(f)$, i.e., $\Theta(\frac{k^*(f)}{\text{poly}(r)})\leq q_t \leq \Theta(k^*(f)\cdot \text{poly}(r))$ and \emph{bad} otherwise. We let $\mathcal{N}_{\good}$ be the collection of elements that arrive at good timesteps. We recall that
\[
k^*(f)= \min_{A\subseteq \calN:\ f(A)<f(\calN)}\left\lfloor \frac{\sum_{e\in \calN}(f(A+e)-f(A))}{f(\calN)-f(A)}\right\rfloor. 
\]
It suffices that dropping all bad elements will not decrease the value of $k^*(f)$ by more than a constant factor, that is,
\begin{equation}
    \frac{\sum_{e\in \mathcal{N}_{\good}} \left(f(A+e)-f(A)\right)}{f(\mathcal{N})-f(A)} =\Omega(k^*(f))\label{equality:technique-target}
\end{equation}
for every set $A\subseteq \mathcal{N}$, since these remaining good elements would contribute to $\Omega(k^*(f)/\log^2 r)$ base colors.

To achieve this, we come to the terminology of quotients in polymatroids. Given a polymatroid $f:2^{\mathcal{N}}\rightarrow \mathbb{Z}_{\geq 0}$ on a ground set $\mathcal{N}$, a quotient is defined to be a set $Q\subseteq \mathcal{N}$ of elements, of which each element has strictly positive merginal function value with respect to $\mathcal{N}\setminus Q$, i.e., $f(e+(\mathcal{N}\setminus Q))>f(\mathcal{N}\setminus Q)$ for every $e\in Q$. The minimum sized quotient is an $r$-approximation of $k^*(f)$ (see Appendix~\ref{section:appendix-quotient}). This guides us to use the minimum sized quotient containing the newly arrived element $e_t$ as the estimate for $k^*(f)$ at timestep $t$ for every $t\in [n]$, that is, 
$$q_t:=\min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}.$$
We note that in the case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$, quotients of $f$ correspond to cut-sets and hence, $q_t$ if the minimum $u_t-v_t$ cut value in graph $(V,E_t)$, where $E_t$ is the collection of the first arrived edges and $u_t, v_t$ are the two end vertices of $e_t$, which is the edge arrives at timestep $t$.

Now, we discuss how to prove equality~(\ref{equality:technique-target}). Fix a set $A\subseteq \mathcal{N}$, we let $T$ be the first timestep that $\frac{\sum_{e\in \mathcal{N}_T}(f(A+e)-f(A))}{f(\mathcal{N})-f(A)}\geq k^*(f)$. We prove that for every timestep $t\in [T]$, our estimation is not too large, that is, $q_t=O(k^*(f)\cdot \text{poly}(r))$. Moreover, based on properties of quotients, we show that for every $j\in \Z_+$, the number of timesteps with $q_t$ being exactly $j$ is at most $r$, which provides an upper bound on the number of timesteps with $q_t=o(k^*(f)/\text{poly}(r))$. This would imply that most of the timesteps $t\in [T]$ are good, which finishes the proof of equality~(\ref{equality:technique-target}). The estimate implies the needed competitive ratio, which indicates that the online arrival order has sufficient information to achieve a $O(\log^2 r)$ competitive ratio.

The rest of the problem is how to get the value of $q_t$ in polynomial time. We note that a $\text{poly}(r)$-approximation of $q_t$ is sufficient since our goal is to estimate $k^*(f)$ within a $\text{poly}(r)$ factor. We achieve this via \emph{strength decomposition} with respect to $f_{|\mathcal{N}_t}$, which is a descending sequence of sets $\mathcal{N}_t=S_0\supseteq S_1\supseteq \ldots \supseteq S_{\ell}=\emptyset$. Let $i\in [0,\ell]$ be the index with $e_t\in S_{i-1}\setminus S_i$. We compute $\eta_t:=\frac{|\mathcal{N}_t\setminus S_i|}{f(\mathcal{N}_t)-f(S_i)}$ and prove that it is an $r$-approximation of $q_t$. See Section~\ref{section:poly-algorithm} for details.

Finally, we consider \DST, which is the special case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$. Our algorithm mentioned above uses the minimum $u_t-v_t$ cut value in graph $(V,E_t)$ as the estimation of $k^*(f)$ at timestep $t$. Indeed, we can use the number of edges connecting $u_t$ and $v_t$ in graph $(V,E_t)$ as an easier estimation. This new estimation still allows us giving an upper bound on the number of timesteps with too small estimation through combinatorial arguments, which implies a faster randomized online algorithm with the same competitive ratio for \DST. The idea for \DCSS is the same as that for \DST. See Section~\ref{section:hypergraph-faster-algo} for details.

==> techniques-2.tex <==
\subsection{Technical Background and Overview of Algorithms}
%\knote{Define quotients, state the estimate, and highlight Lemma \ref{lemma:counting-quotient} as the novel structural property. Explain how the lemma is useful to design an online algorithm with polylog competitive ratio.}
%\cnote{I think this is too long. We need to say something about estimating the $k_t$ approximately. It would be useful to discuss disjoint set covers and briefly say that we are inspired by trying to abstract out that approach and do it via quotients. I think that is sufficient, especially for the confence version where we are going to have space limitations.} \cnote{Update: I still think this is too long. We are giving a fairly detailed informal description of the algorithm and we only have 15 pages. Change the title to "Overview of the Algorithms" if we keep this level of detail. It seems that some definitions are moved to this section. We have to be careful in case some reader skips this section. Perhaps we should say "Technical background and overview of algorithms". I am fine with whatever decision you make. }
\iffalse
Let us first consider \DSC, where the polymatroid $f$ is defined to be the coverage function of the input hypergraph $H=(V,E)$. We let $n:=|V|$ be the number of vertices and $m:=|E|$ be the number of hyperedges. As we have mentioned before, the quantity $k^*$ equals the min-degree $\delta_H$ of $H$. If the min-degree $\delta_H$ is known in advance, Pananjady, Bagaria, and Vaze \cite{PBV15} showed that sampling the color of each hypergraph uniformly from the palette $[\Theta(\delta_H/\log n)]$ would lead to $\Omega(\delta_H/\log n)$ base colors. Emek, Goldbraikh, and Kantor \cite{EGK19} presented a randomized online algorithm without prior knowledge of $\delta_H$. Their algorithm works as follows: When hyperedge $e_t$ arrives, the algorithm first computes the min-degree $\delta_t$ of a vertex in $e_t$ in the hypergraph containing all hyperedges that have arrives so far. By a combinatorial lemma, they showed that $\delta_t\leq \delta_H\leq \delta_t\cdot O(n)$ for a constant fraction of timesteps $t\in [m]$. Their algorithm then 
%guesses the value of $\delta$ by sampling 
samples 
$P_t$ uniformly from $\{\delta_t\cdot 2^0, \delta_t\cdot 2^1, \delta_t\cdot 2^2, \ldots, \delta_t\cdot 2^{O(\log n)}\}$. We note that if $\delta_t\le \delta_H\le \delta_t\cdot O(n)$, then $P_t$ is a $2$-approximation of $\delta_H$ with probability $\Omega(\frac{1}{\log n})$. Finally, the algorithm samples the color $C(e_t)$ of the hyperedge $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 n)]$. Since expected $\Omega(1/\log n)$ fraction of timesteps obtain a $2$-approximation of $\delta_H$, the algorithm achieves $\Omega(\delta_H/\log ^2n)$ base colors in expectation. We note that $\opt(f)\le k^* = \delta_H$ and hence the competitive ratio is $O(\log^2 n)$. 
\fi

%In this work, our main contribution is appropriately generalizing the above ideas to \DPB. 
Let $f:2^\mathcal{N} \rightarrow \Z_{\ge 0}$ be the polymatroid of interest. Let  $r:=f(\mathcal{N})$ be the function value of bases and $k^*:=k^*(f)$. For the discussion here, we will assume that $f(e)>0$ for every $e\in \calN$, $r\geq 2$, and $k^*=\Omega(\log^2 r)$ since this is the non-trivial case. 
%(this assumption can be relaxed by combining the algorithm for this case with those designed for other cases---see Section~\ref{subsection:mixed-algorithm}). 
First consider the setting where the online algorithm knows $k^*$ in advance. In this setting, coloring each element uniformly from the palette $[\Theta(k^*/\log r)]$ gives $\Omega(k^*/\log{r})$ base colors, thereby leading to a $O(\log{r})$-competitive ratio. 
%This follows from previous work in \cite{CCV09}, but we give an alternative proof since we will require this alternative viewpoint for our purposes:  We show that 
This is because a random subset obtained by picking each element in $\mathcal{N}$ with probability $\Omega(\log r/k^*)$ independently at random is a base with constant probability---see Lemma~\ref{lemma:sampling-property}. %Hence, every color in the palette is a base color with constant probability, which implies that the random coloring algorithm will attain $\Omega(k^*/\log r)$ base colors in expectation.

Next, consider the setting of interest, namely $k^*$ is not known in advance. In this setting, our approach is to \emph{estimate} $k^*$ at each timestep. 
%Adapting the idea used in \DSC, our algorithm has the following framework: 
%When element $e_t$ arrives, suppose that we can estimate $q_t$ of $k^*$. 
At each timestep $t\in [n]$, suppose that we can 
estimate $q_t$ within a $\text{poly}(r)$ factor of $k^*$---we 
%compute an \emph{estimate} $q_t$ that is within a $\text{poly}(r)$ factor of $k^*$, that is, $\Theta\left(\frac{k^*}{\text{poly}(r)}\right)\leq q_t \leq \Theta(k^*\cdot \text{poly}(r))$---we 
call such an estimate to be a \emph{coarse estimate}. 
We can fine-tune such a coarse estimate by randomization as follows: sample $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$, where $q_t$ is the coarst estimate; we note that $P_t$ is a $2$-approximation of $k^*$ with probability $\Omega(1/\log r)$. Consequently, 
%we can obtain a $2$-approximation $P_t$ of $k^*$ with probability $\Omega(1/\log r)$ by sampling $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$. In this way, 
coloring the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$ would lead to $\Omega(k^*/ \log^2 r)$ base colors in 
expectation (using the arguments in the previous paragraph). 
%expectation. This is because, for a fixed color $c\in [\Theta(k^*)/\log^2{r}]$, each element is colored $c$ with probability $\Omega(\log{r}/k^*)$. Thus, each color in $[\Theta(k^*)/\log^2{r}]$ is a base color with constant probability (using the arguments in the previous paragraph) and hence, the expected number of base colors is $\Omega(k^*/ \log^2 r)$. 
In summary, a coarse estimate for $k^*$ at each timestep suffices to achieve a $O(\log^2{r})$-competitive ratio. We emphasize that we rely on randomization only to fine-tune the coarse estimate and to perform random coloring. The rest of our techniques will not involve randomization. 

Based on the discussion in the previous paragraph, the key challenge is computing a coarse estimate for $k^*$ using limited knowledge of the polymatroid (restricted to the elements that have arrived so far). 
We do not know how to compute a coarse estimate for $k^*$ in \emph{all} timesteps given the limited knowledge of the polymatroid.  
%(we also do not know if a coarse estimate in a constant fraction of timesteps suffices or even how to compute a coarse estimate at a constant fraction of timesteps). 
Instead, we compute an estimate at each timestep such that the elements at timesteps which achieve the coarse property provide \emph{a sufficiently large value of $k^*$}. We formalize this approach now. 
%However, we will compute a coarse estimate for $k^*$ in \emph{a sufficiently large number of timesteps} \knote{This is not about sufficiently large number of timesteps. Could explain better.}. 
%Although we do not know how to estimate $k^*$ within a $\text{poly}(r)$ factor, we will achieve this for enough timesteps. 
Suppose we have a subroutine to compute some estimate $q_t$ at each timestep $t\in [n]$ using limited knowledge of the polymatroid. Let us understand the properties needed from the estimator in order to achieve $\Omega(k^*/\log^2{r})$ base colors via the 
%random sampling followed by 
fine-tuned random coloring argument from the previous paragraph. 
We call a timestep $t\in [n]$ to be \emph{good} if the estimate $q_t$ is a coarse estimate of $k^*$ and \emph{bad} otherwise.
%For a timestep $t\in [n]$, we call it a \emph{good} timestep if our estimate $q_t$ is within a $\text{poly}(r)$ factor of $k^*$, i.e., $\Theta(\frac{k^*}{\text{poly}(r)})\leq q_t \leq \Theta(k^*\cdot \text{poly}(r))$ and \emph{bad} otherwise. 
We note that the online algorithm does not have to verify whether a timestep is good or bad (i.e., whether the estimate at a timestep is coarse) and that these notions are used only for the purpose of the analysis. 
We let $\mathcal{N}_{\good}$ be the collection of elements that arrive at good timesteps. 
\iffalse
We recall that 
\begin{align*}
k^*&= \min_{A\subseteq \calN:\ f(A)<f(\calN)} \left \lfloor\frac{\sum_{e\in \calN}(f(A+e)-f(A))}{f(\calN)-f(A)}\right \rfloor. 
\end{align*}
\fi
An equivalent interpretation of $k^*$ is the following: 
\begin{align}
    k^* &= \max\left\{k\in \Z_{\ge 0}: \sum_{e\in \calN}\left(f(A+e)-f(A)\right) \ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN\right\}. 
    %\sum_{e\in \calN}\left((f(A+e)-f(A)\right) &\ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN
    \label{equality:technique-alternative-intepretation-k*}
\end{align}
Suppose that our estimator subroutine can guarantee the following property: %for some $k=\Omega(k^*)$: 
%\begin{align}
%    \sum_{e\in \calN_{\good}}(f(A+e)-f(A)) &\ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN
%    \label{equality:technique-target}
%\end{align}
\begin{align}
    k_{\text{onl}}^* &:= \max\left\{k\in \Z_{\ge 0}: \sum_{e\in \calN_{\good}}(f(A+e)-f(A)) \ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN \right\}=\Omega(k^*).
    \label{equality:technique-target}
\end{align}
Note the difference in the definition of $k_\text{onl}^*$ and $k^*$: the definition of $k^*$ takes the sum of marginals of all elements while the definition of $k_\text{onl}^*$ focuses on the sum of marginals of only good elements. Moreover, the definition $k_\text{onl}^*$ depends on the set of good elements, which in turn, depends on the estimate $q_t$. 
%LHS of \eqref{equality:technique-alternative-intepretation-k*} and \eqref{equality:technique-target}. 
The property $k_\text{onl}^*=\Omega(k^*)$ mentioned in \eqref{equality:technique-target} essentially says that dropping the bad elements in the definition of $k^*$ does not decrease $k^*$ by more than a constant factor. 
\iffalse
One consequence of property \ref{equality:technique-target} is that (apply the property for $A=\calN_{\good}$)
\begin{align}
    f(\calN_{\good})=f(\calN). 
\end{align} 
\fi
Property \eqref{equality:technique-target} suffices to obtain $\Omega(k^*/\log^2{r})$ base colors in expectation via the fine-tuned random coloring argument in the previous paragraph: sample $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$ and color the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$. 
For the analysis, we focus on the polymatroid $f$ restricted to good elements, i.e., $f_{|\calN_{\good}}$; we note that bases of $f_{|\calN_{\good}}$ are also bases of $f$ since $f(\calN_{\good})=f(\calN)$ (by applying property \eqref{equality:technique-target} to $A=\calN_{\good}$). 
We observe that for a fixed color $c\in [\Theta(k^*)/\log^2{r}]$, each ``good'' element is colored $c$ with probability $\Omega(\log{r}/k_\text{onl})=\Omega(\log{r}/k^*)$. Hence, using the analysis mentioned in the second paragraph to the polymatroid $f_{|\calN_{\good}}$ shows that the algorithm returns $\Omega(k^*/\log^2{r})$ base colors of $f_{|\calN_{\good}}$ and consequently of $f$, in expectation---see Lemma \ref{lemma:polymatroid-proper-color-probability} for details. 

In order to design an estimator $q_t$ that achieves the property mentioned in \eqref{equality:technique-target}, we rely on the notion of \emph{quotients}. 
\begin{definition}\label{defn:quotients}
For a polymatroid $g:2^{\mathcal{V}}\rightarrow \mathbb{Z}_{\geq 0}$ on a ground set $\mathcal{V}$, a set $Q\subseteq \mathcal{V}$ is a \emph{quotient} of $g$ if $g(e+(\mathcal{V}\setminus Q))>g(\mathcal{V}\setminus Q)$ for every $e\in Q$, i.e., if each element $e\in Q$ has strictly positive marginal with respect to $\mathcal{V}\setminus Q$. 
\end{definition}
Since the definition of quotients might seem contrived, we interpret it for some concrete polymatroids: 
\begin{enumerate}
\item Let $G=(V, E)$ be a connected hypergraph (graph respectively). Consider the polymatroid $g:2^E\rightarrow \Z_{\ge 0}$ that arises in \DCSS (\DST respectively) with $G$ being the input instance. Quotients of $g$ correspond to union of cut-set of disjoint subsets of vertices, i.e., each quotient $Q\subseteq E$ of $g$ is of the form $Q=\cup_{S\in \mathcal{C}}\delta(S)$, where the family $\mathcal{C}\subseteq 2^V\setminus \{\emptyset, V\}$ is a disjoint family of subsets of vertices. In particular, the minimum size of a non-empty quotient is equal to the global min-cut value of $G$. 
\item Let $G=(V, E)$ be a hypergraph. Consider the polymatroid $g: 2^E\rightarrow \Z_{\ge 0}$ that arises in \DSC with $G$ being the input instance, i.e., $g$ is the coverage function of $G$. Quotients of $g$ correspond to union of vertex-isolating cuts of $G$, i.e., each quotient $Q\subseteq E$ of $g$ is of the form $Q=\cup_{u\in S}\delta(u)$ where  $S\subseteq V$. In particular, the minimum size of a non-empty quotient is equal to the min-degree of $G$. %\knote{@Weihao, Verify this and release this comment after confirming.}
\end{enumerate}


We observed that the minimum size of a non-empty quotient of $f$ is an $r$-approximation of $k^*$---see Appendix~\ref{section:appendix-quotient}. This inspired us to use the minimum-sized quotient of $f_{|\calN_t}$ that \emph{contains $e_t$} as the estimate at each timestep $t\in [n]$. That is, we use the estimator defined as 
\begin{align}\label{techniques:estimate-q_t}
    q_t&:=\min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}.
\end{align}
We use this estimator followed by fine-tuned random coloring as our randomized online algorithm---see 
%We state the algorithm based on this estimator in 
Algorithm \ref{algo:pseudocode-polymatroid}. 
%We note that in the case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$, quotients of $f$ correspond to cut-sets and hence, $q_t$ is the minimum $u_t-v_t$ cut value in the graph $(V,E_t)$, where $E_t$ is the set of edges that have arrived until time $t$ and $u_t, v_t$ are the end vertices of the edge $e_t$ that arrives at timestep $t$.
Now, we outline how to conclude the property mentioned in \eqref{equality:technique-target} using the estimate $q_t$ given in \eqref{techniques:estimate-q_t} at each timestep $t\in [n]$. Fix an arbitrary set $A\subseteq \mathcal{N}$. We need to show that $\sum_{e\in \calN_{\good}}(f(A+e)-f(A))=\Omega(k^*)(f(\calN)-f(A))$. 
We note that $\sum_{e\in \mathcal{N}_t}(f(A+e)-f(A))$ is non-decreasing with $t$ owing to monotonicity. Let $T$ be the first timestep such that $\sum_{e\in \mathcal{N}_T}(f(A+e)-f(A))\ge k^* (f(\mathcal{N})-f(A))$. We prove that for every timestep $t\in [T]$, our estimator is not too large, that is, $q_t=O(k^*\cdot \text{poly}(r))$---see Lemma \ref{lemma:q_t-upper-bound}. Consequently, the only reason for an element $e_t$ to be bad is that the estimate $q_t$ is too small. As a main structural property of polymatroids, we show that for every $j\in \Z_+$, the number of timesteps $t$ with $q_t$ being exactly $j$ is at most $r$---see Lemma \ref{lemma:counting-quotient}. This structural property is a general statement about a polymatroid with respect to an arbitrary ordering and we believe that it could have other implications. A consequence of this structural property is that the number of timesteps $t$ with small $q_t$ is small---e.g., the number of timesteps $t$ with $q_t\le k^*/2r$ is at most $k^*/2$. Hence, at least $T-k^*/2$ timesteps $t\in [T]$ are good; we use this fact to conclude that $\sum_{e\in \calN_{\good}}(f(A+e)-f(A))=\Omega(k^*)(f(\calN)-f(A))$---see Lemma \ref{lemma:new-ratio-closed}, Corollary \ref{corollary:new-ratio}, and Lemma \ref{lemma:new-opt}. Thus, the estimate achieves property \eqref{equality:technique-target} which leads to the stated competitive ratio. 

The main takeaway from Algorithm \ref{algo:pseudocode-polymatroid} using the estimator $q_t$ given in \eqref{techniques:estimate-q_t} and its analysis is that the online arrival order has sufficient information to achieve an $O(\log^2 r)$ competitive ratio. We will discuss the runtime issue of Algorithm \ref{algo:pseudocode-polymatroid} shortly. We mention that our Algorithm \ref{algo:pseudocode-polymatroid} and its analysis specialized for coverage functions correspond to the algorithm of Emek, Goldbraikh, and Kantor for \DSC \cite{EGK19}. Thus, one of our contributions is appropriately generalizing their algorithm and analysis from \DSC to the more general case of \DPB.  

Now, we address the runtime of Algorithm \ref{algo:pseudocode-polymatroid}. We observe that the quantity $q_t$ is NP-hard to compute. 
%The problem of computing a min-sized non-empty quotient of a polymatroid is NP-hard. This is because, a min-sized quotient of a matroid is equal to the cogirth of the matroid which is NP-hard to compute \cite{Var97}. It is easy to see that cogirth of a matroid reduces to computing $q_t$ and hence, $q_t$ is NP-hard to compute. 
%For this reason, we believe that the estimate $q_t$ is not likely to be computable in polynomial time. 
%The next issue is how to compute the value of $q_t$ in polynomial time. 
However, we note that a $\text{poly}(r)$-approximation of $q_t$ is sufficient for the desired competitive ratio since our goal is to estimate $k^*$ within a $\text{poly}(r)$ factor. We show that an $r$-approximation of $q_t$ can be computed using a \emph{strength decomposition} with respect to $f_{|\mathcal{N}_t}$. 
%, which is a descending sequence of sets $\mathcal{N}_t=S_0\supseteq S_1\supseteq \ldots \supseteq S_w=\emptyset$. Let $i\in [0,w]$ be the index with $e_t\in S_{i-1}\setminus S_i$. We compute $$\eta_t:=\frac{|\mathcal{N}_t\setminus S_i|}{f(\mathcal{N}_t)-f(S_i)}$$ and prove that it is an $r$-approximation of $q_t$. 
See Algorithm \ref{algo:pseudocode-polymatroid-polynomial} and its analysis in Section~\ref{section:poly-algorithm} which completes the proof of Theorem \ref{main-result:polymatroid}.

Finally, we outline our simpler algorithm for \DCSS and \DST mentioned in Theorem \ref{main-result:hypergaph}. For simplicity, we will focus on \DST here. The polymatroid $f:2^E\rightarrow \Z_{\ge 0}$ of interest here is the rank function of the graphic matroid defined by the undirected graph $G=(V, E)$. Our Algorithm \ref{algo:pseudocode-polymatroid} for this polymatroid can be implemented in polynomial-time since the estimate $q_t$ is equal to the min $u_t-v_t$ cut value in the graph $(V, E_t)$ containing all edges that have arrived so far. We recall that min $u_t-v_t$ cut can be computed in polynomial time via one application of max flow. However, we show that a much simpler estimator for \DST also achieves the property mentioned in \eqref{equality:technique-target}: we use 
\[
\eta_t:= \text{number of edges between $u_t$ and $v_t$ in the graph $(V, E_t)$}
\]
where $u_t$ and $v_t$ are the end vertices of the edge $e_t$ that arrives at time $t$. Our proof that this estimator achieves the property mentioned in \eqref{equality:technique-target} is via combinatorial arguments and it also generalizes to \DCSS. See Section \ref{section:hypergraph-faster-algo} for details. 

%Finally, we consider \DST, which is the special case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$. Our algorithm mentioned above uses the minimum $u_t-v_t$ cut value in graph $(V,E_t)$ as the estimation of $k^*$ at timestep $t$. Indeed, we can use the number of edges connecting $u_t$ and $v_t$ in graph $(V,E_t)$ as an easier estimation. This new estimation still allows us giving an upper bound on the number of timesteps with too small estimation through combinatorial arguments, which implies a faster randomized online algorithm with the same competitive ratio for \DST. The idea for \DCSS is the same as that for \DST. See Section~\ref{section:hypergraph-faster-algo} for details.

==> techniques-3.tex <==
\subsection{Technical Background and Overview of Algorithms}
\znote{This is the long version of techniques section. See the short version in techniques-short-version.tex.}
%\knote{Edited this section. Proofread.}
%\knote{Define quotients, state the estimate, and highlight Lemma \ref{lemma:counting-quotient} as the novel structural property. Explain how the lemma is useful to design an online algorithm with polylog competitive ratio.}
%\cnote{I think this is too long. We need to say something about estimating the $k_t$ approximately. It would be useful to discuss disjoint set covers and briefly say that we are inspired by trying to abstract out that approach and do it via quotients. I think that is sufficient, especially for the confence version where we are going to have space limitations.} \cnote{Update: I still think this is too long. We are giving a fairly detailed informal description of the algorithm and we only have 15 pages. Change the title to "Overview of the Algorithms" if we keep this level of detail. It seems that some definitions are moved to this section. We have to be careful in case some reader skips this section. Perhaps we should say "Technical background and overview of algorithms". I am fine with whatever decision you make. }
\iffalse
Let us first consider \DSC, where the polymatroid $f$ is defined to be the coverage function of the input hypergraph $H=(V,E)$. We let $n:=|V|$ be the number of vertices and $m:=|E|$ be the number of hyperedges. As we have mentioned before, the quantity $k^*$ equals the min-degree $\delta_H$ of $H$. If the min-degree $\delta_H$ is known in advance, Pananjady, Bagaria, and Vaze \cite{PBV15} showed that sampling the color of each hypergraph uniformly from the palette $[\Theta(\delta_H/\log n)]$ would lead to $\Omega(\delta_H/\log n)$ base colors. Emek, Goldbraikh, and Kantor \cite{EGK19} presented a randomized online algorithm without prior knowledge of $\delta_H$. Their algorithm works as follows: When hyperedge $e_t$ arrives, the algorithm first computes the min-degree $\delta_t$ of a vertex in $e_t$ in the hypergraph containing all hyperedges that have arrives so far. By a combinatorial lemma, they showed that $\delta_t\leq \delta_H\leq \delta_t\cdot O(n)$ for a constant fraction of timesteps $t\in [m]$. Their algorithm then 
%guesses the value of $\delta$ by sampling 
samples 
$P_t$ uniformly from $\{\delta_t\cdot 2^0, \delta_t\cdot 2^1, \delta_t\cdot 2^2, \ldots, \delta_t\cdot 2^{O(\log n)}\}$. We note that if $\delta_t\le \delta_H\le \delta_t\cdot O(n)$, then $P_t$ is a $2$-approximation of $\delta_H$ with probability $\Omega(\frac{1}{\log n})$. Finally, the algorithm samples the color $C(e_t)$ of the hyperedge $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 n)]$. Since expected $\Omega(1/\log n)$ fraction of timesteps obtain a $2$-approximation of $\delta_H$, the algorithm achieves $\Omega(\delta_H/\log ^2n)$ base colors in expectation. We note that $\opt(f)\le k^* = \delta_H$ and hence the competitive ratio is $O(\log^2 n)$. 
\fi

%In this work, our main contribution is appropriately generalizing the above ideas to \DPB. 
We recall that we assume $\mathcal{N}$ is the input sequence. Let $f:2^\mathcal{N} \rightarrow \Z_{\ge 0}$ be the polymatroid of interest. Let  $r:=f(\mathcal{N})$ be the function value of bases and $k^*:=k^*(f)$. For the discussion here, we will assume that $f(e)>0$ for every $e\in \calN$, $r\geq 2$, and $k^*=\Omega(\log^2 r)$ since this is the non-trivial case. 
%(this assumption can be relaxed by combining the algorithm for this case with those designed for other cases---see Section~\ref{subsection:mixed-algorithm}). 
First consider the setting where the online algorithm knows $k^*$ in advance. In this setting, coloring each element uniformly from the palette $[\Theta(k^*/\log r)]$ gives $\Omega(k^*/\log{r})$ base colors, thereby leading to an $O(\log{r})$-competitive ratio. 
%This follows from previous work in \cite{CCV09}, but we give an alternative proof since we will require this alternative viewpoint for our purposes:  We show that 
This is because a random subset obtained by picking each element in $\mathcal{N}$ with probability $\Omega(\log r/k^*)$ independently at random is a base with constant probability---see Lemma~\ref{lemma:sampling-property}. %Hence, every color in the palette is a base color with constant probability, which implies that the random coloring algorithm will attain $\Omega(k^*/\log r)$ base colors in expectation.

Next, consider the setting of interest, namely $k^*$ is not known in advance. In this setting, our approach is to \emph{estimate} $k^*$ at each timestep. 
%Adapting the idea used in \DSC, our algorithm has the following framework: 
%When element $e_t$ arrives, suppose that we can estimate $q_t$ of $k^*$. 
At each timestep $t\in [n]$, suppose that we can 
estimate $q_t$ within a $\text{poly}(r)$ factor of $k^*$, i.e., $q_t\in [\frac{k^*}{\text{poly}(r)}, k^*\cdot \text{poly}(r)]$, then we 
%compute an \emph{estimate} $q_t$ that is within a $\text{poly}(r)$ factor of $k^*$, that is, $\Theta\left(\frac{k^*}{\text{poly}(r)}\right)\leq q_t \leq \Theta(k^*\cdot \text{poly}(r))$---we 
call such an estimate to be a \emph{coarse estimate}. 
We can fine-tune such a coarse estimate by randomization as follows: sample $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$, where $q_t$ is the coarst estimate; we note that $P_t$ is a $2$-approximation of $k^*$ with probability $\Omega(1/\log r)$. Consequently, 
%we can obtain a $2$-approximation $P_t$ of $k^*$ with probability $\Omega(1/\log r)$ by sampling $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$. In this way, 
coloring the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$ would lead to $\Omega(k^*/ \log^2 r)$ base colors in 
expectation (using the arguments in the previous paragraph). 
%expectation. This is because, for a fixed color $c\in [\Theta(k^*)/\log^2{r}]$, each element is colored $c$ with probability $\Omega(\log{r}/k^*)$. Thus, each color in $[\Theta(k^*)/\log^2{r}]$ is a base color with constant probability (using the arguments in the previous paragraph) and hence, the expected number of base colors is $\Omega(k^*/ \log^2 r)$. 
In summary, a coarse estimate for $k^*$ at each timestep suffices to achieve an $O(\log^2{r})$-competitive ratio. We emphasize that we rely on randomization only to fine-tune the coarse estimate and to perform random coloring. The rest of our techniques will not involve randomization. 

Based on the discussion in the previous paragraph, the key challenge is computing a coarse estimate for $k^*$ using limited knowledge of the polymatroid (restricted to the elements that have arrived so far). 
We do not know how to compute a coarse estimate for $k^*$ at \emph{all} timesteps given the limited knowledge of the polymatroid.  
%(we also do not know if a coarse estimate in a constant fraction of timesteps suffices or even how to compute a coarse estimate at a constant fraction of timesteps). 
Instead, we compute an estimate at each timestep such that the elements at timesteps which achieve the coarse property provide \emph{a sufficiently large value of $k^*$}. We formalize this approach now. 
%However, we will compute a coarse estimate for $k^*$ in \emph{a sufficiently large number of timesteps} \knote{This is not about sufficiently large number of timesteps. Could explain better.}. 
%Although we do not know how to estimate $k^*$ within a $\text{poly}(r)$ factor, we will achieve this for enough timesteps. 
Suppose we have a subroutine to compute some estimate $q_t$ at each timestep $t\in [n]$ using limited knowledge of the polymatroid. Let us understand the properties needed from the estimator in order to achieve $\Omega(k^*/\log^2{r})$ base colors via the 
%random sampling followed by 
fine-tuned random coloring argument from the previous paragraph. 
We call a timestep $t\in [n]$ to be \emph{good} if the estimate $q_t$ is a coarse estimate of $k^*$ and \emph{bad} otherwise.
%For a timestep $t\in [n]$, we call it a \emph{good} timestep if our estimate $q_t$ is within a $\text{poly}(r)$ factor of $k^*$, i.e., $\Theta(\frac{k^*}{\text{poly}(r)})\leq q_t \leq \Theta(k^*\cdot \text{poly}(r))$ and \emph{bad} otherwise. 
We note that the online algorithm does not have to verify whether a timestep is good or bad (i.e., whether the estimate at a timestep is coarse) and that these notions are used only for the purpose of the analysis. 
We let $\mathcal{N}_{\good}$ be the collection of elements that arrive at good timesteps and focus on the function $f$ restricted to $\calN_{\good}$, i.e., on the function $g:=f_{|\calN_{\good}}$. Suppose that the following two properties hold:
\begin{enumerate}[label=(\roman*)]
    \item Bases of $g$ are also bases of $f$ and 
    \item $k^*(g)=\Omega(1) k^*$, i.e., the quantity $k^*$ for the function $f$ restricted to good elements is at least a constant fraction of $k^*$ for the function $f$ itself. 
\end{enumerate}
These two properties suffice to obtain $\Omega(k^*/\log^2{r})$ base colors in expectation via the fine-tuned random coloring argument in the previous paragraph: sample $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$ and color the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$. 
For the analysis, we focus on the polymatroid $f$ restricted to good elements, i.e., $f_{|\calN_{\good}}$; we note that bases of $f_{|\calN_{\good}}$ are also bases of $f$ by property (i). 
We observe that for a fixed color $c\in [\Theta(k^*)/\log^2{r}]$, each ``good'' element is colored $c$ with probability $\Omega(\log{r}/k^*)=\Omega(\log{r}/k^*(g))$, where the last equation is by property (ii). Hence, using the analysis mentioned in the second paragraph for the polymatroid $f_{|\calN_{\good}}$ shows that the algorithm returns $\Omega(k^*/\log^2{r})$ base colors of $f_{|\calN_{\good}}$ and consequently of $f$, in expectation---see Lemma \ref{lemma:polymatroid-proper-color-probability} for details. 
\iffalse
We recall that 
\begin{align*}
k^*&= \min_{A\subseteq \calN:\ f(A)<f(\calN)} \left \lfloor\frac{\sum_{e\in \calN}(f(A+e)-f(A))}{f(\calN)-f(A)}\right \rfloor. 
\end{align*}
\fi
\iffalse
An equivalent interpretation of $k^*$ is the following: 
\begin{align}
    k^* &= \max\left\{k\in \Z_{\ge 0}: \sum_{e\in \calN}\left(f(A+e)-f(A)\right) \ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN\right\}. 
    %\sum_{e\in \calN}\left((f(A+e)-f(A)\right) &\ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN
    \label{equality:technique-alternative-intepretation-k*}
\end{align}
Suppose that our estimator subroutine can guarantee the following property: %for some $k=\Omega(k^*)$: 
%\begin{align}
%    \sum_{e\in \calN_{\good}}(f(A+e)-f(A)) &\ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN
%    \label{equality:technique-target}
%\end{align}
\begin{align}
    k_{\text{onl}}^* &:= \max\left\{k\in \Z_{\ge 0}: \sum_{e\in \calN_{\good}}(f(A+e)-f(A)) \ge k(f(\calN)-f(A))\ \forall\ A\subseteq \calN \right\}=\Omega(k^*).
    \label{equality:technique-target}
\end{align}
Note the difference in the definition of $k_\text{onl}^*$ and $k^*$: the definition of $k^*$ takes the sum of marginals of all elements while the definition of $k_\text{onl}^*$ focuses on the sum of marginals of only good elements. Moreover, the definition $k_\text{onl}^*$ depends on the set of good elements, which in turn, depends on the estimate $q_t$. 
%LHS of \eqref{equality:technique-alternative-intepretation-k*} and \eqref{equality:technique-target}. 
The property $k_\text{onl}^*=\Omega(k^*)$ mentioned in \eqref{equality:technique-target} essentially says that dropping the bad elements in the definition of $k^*$ does not decrease $k^*$ by more than a constant factor. 
\iffalse
One consequence of property \ref{equality:technique-target} is that (apply the property for $A=\calN_{\good}$)
\begin{align}
    f(\calN_{\good})=f(\calN). 
\end{align} 
\fi
Property \eqref{equality:technique-target} suffices to obtain $\Omega(k^*/\log^2{r})$ base colors in expectation via the fine-tuned random coloring argument in the previous paragraph: sample $P_t$ uniformly from $\{q_t\cdot 2^{-O(\log r)}, \ldots, q_t\cdot 2^{-1}, q_t\cdot 2^0, q_t\cdot 2^{1}, \ldots, q_t\cdot 2^{O(\log r)}\}$ and color the element $e_t$ uniformly from the palette $[\Theta(P_t/\log^2 r)]$. 
For the analysis, we focus on the polymatroid $f$ restricted to good elements, i.e., $f_{|\calN_{\good}}$; we note that bases of $f_{|\calN_{\good}}$ are also bases of $f$ since $f(\calN_{\good})=f(\calN)$ (by applying property \eqref{equality:technique-target} to $A=\calN_{\good}$). 
We observe that for a fixed color $c\in [\Theta(k^*)/\log^2{r}]$, each ``good'' element is colored $c$ with probability $\Omega(\log{r}/k_\text{onl})=\Omega(\log{r}/k^*)$. Hence, using the analysis mentioned in the second paragraph to the polymatroid $f_{|\calN_{\good}}$ shows that the algorithm returns $\Omega(k^*/\log^2{r})$ base colors of $f_{|\calN_{\good}}$ and consequently of $f$, in expectation---see Lemma \ref{lemma:polymatroid-proper-color-probability} for details. 
\fi

In order to design an estimator $q_t$ that achieves the two properties mentioned above, we rely on the notion of \emph{quotients}. 
\begin{definition}\label{defn:quotients}
For a polymatroid $h:2^{\mathcal{V}}\rightarrow \mathbb{Z}_{\geq 0}$ on a ground set $\mathcal{V}$, a set $Q\subseteq \mathcal{V}$ is a \emph{quotient} of $h$ if $h(e+(\mathcal{V}\setminus Q))>h(\mathcal{V}\setminus Q)$ for every $e\in Q$, i.e., if each element $e\in Q$ has strictly positive marginal with respect to $\mathcal{V}\setminus Q$. 
\end{definition}
Since the definition of quotients might seem contrived, we interpret it for some concrete polymatroids: 
\begin{enumerate}
\item Let $G=(V, E)$ be a connected hypergraph (graph respectively). Consider the polymatroid $h:2^E\rightarrow \Z_{\ge 0}$ that arises in \DCSS (\DST respectively) with $G$ being the input instance. Quotients of $h$ correspond to union of cut-set of disjoint subsets of vertices, i.e., each quotient $Q\subseteq E$ of $h$ is of the form $Q=\cup_{S\in \mathcal{C}}\delta(S)$, where the family $\mathcal{C}\subseteq 2^V\setminus \{\emptyset, V\}$ is a disjoint family of subsets of vertices. In particular, the minimum size of a non-empty quotient is equal to the global min-cut value of $G$. 
\item Let $G=(V, E)$ be a hypergraph. Consider the polymatroid $h: 2^E\rightarrow \Z_{\ge 0}$ that arises in \DSC with $G$ being the input instance, i.e., $h$ is the coverage function of $G$. Quotients of $h$ correspond to union of vertex-isolating cuts of $G$, i.e., each quotient $Q\subseteq E$ of $h$ is of the form $Q=\cup_{u\in S}\delta(u)$ where  $S\subseteq V$. In particular, the minimum size of a non-empty quotient is equal to the min-degree of $G$. %\knote{@Weihao, Verify this and release this comment after confirming.}
\end{enumerate}


We observed that the minimum size of a non-empty quotient of $f$ is an $r$-approximation of $k^*$---see Appendix~\ref{section:appendix-quotient}. This inspired us to use the minimum-sized quotient of $f_{|\calN_t}$ that \emph{contains $e_t$} as the estimate at each timestep $t\in [n]$. That is, we use the estimator defined as 
\begin{align}\label{techniques:estimate-q_t}
    q_t&:=\min \{|Q|: e_t\in Q \subseteq \mathcal{N}_t \text{ and $Q$ is a quotient of $f_{|\mathcal{N}_t}$}\}.
\end{align}
We use this estimator followed by fine-tuned random coloring as our randomized online algorithm---see 
%We state the algorithm based on this estimator in 
Algorithm \ref{algo:pseudocode-polymatroid}. 
%We note that in the case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$, quotients of $f$ correspond to cut-sets and hence, $q_t$ is the minimum $u_t-v_t$ cut value in the graph $(V,E_t)$, where $E_t$ is the set of edges that have arrived until time $t$ and $u_t, v_t$ are the end vertices of the edge $e_t$ that arrives at timestep $t$.

Now, we outline how to conclude the properties (i) and (ii) mentioned above using the estimate $q_t$ given in \eqref{techniques:estimate-q_t} for each timestep $t\in [n]$. We will show that 
\begin{equation}
\sum_{e\in \calN_{\good}} (f(A+e)-f(A))\ge \Omega(k^*)(f(\calN)-f(A)) \ \forall\ A\subseteq \calN. \label{eq:techniques}
\end{equation}
This implies both properties: property (i) follows by applying the inequality in \eqref{eq:techniques} to the set $A=\calN_{\good}$, using $k^*>0$, and concluding that $f(\calN_{\good})=f(\calN)$; property (ii) follows from reinterpreting property (i) as saying that $f(\calN)=f(\calN_{\good})$, the inequalities in \eqref{eq:techniques}, and the definition of $k^*(g)$. 
We now sketch our proof of \eqref{eq:techniques}. 
Fix an arbitrary set $A\subseteq \mathcal{N}$. We need to show that $\sum_{e\in \calN_{\good}}(f(A+e)-f(A))=\Omega(k^*)(f(\calN)-f(A))$. 
We note that $\sum_{e\in \mathcal{N}_t}(f(A+e)-f(A))$ is non-decreasing with $t$ owing to monotonicity. Let $T$ be the first timestep such that $\sum_{e\in \mathcal{N}_T}(f(A+e)-f(A))\ge k^* (f(\mathcal{N})-f(A))$. We prove that for every timestep $t\in [T]$, our estimator is not too large, that is, $q_t=O(k^*\cdot \text{poly}(r))$---see Lemma \ref{lemma:q_t-upper-bound}. Consequently, the only reason for an element $e_t$ with $t\in [T]$ to be bad is that the estimate $q_t$ is too small. As a main structural property of polymatroids, we show that for every $j\in \Z_+$, the number of timesteps $t$ with $q_t$ being exactly $j$ is at most $r$---see Lemma \ref{lemma:counting-quotient}. This structural property is a general statement about a polymatroid with respect to an arbitrary ordering and we believe that it could have other implications. A consequence of this structural property is that the number of timesteps $t$ with small $q_t$ is small---e.g., the number of timesteps $t$ with $q_t\le k^*/2r$ is at most $k^*/2$. Hence, at least $T-k^*/2$ timesteps $t\in [T]$ are good; we use this fact to conclude that $\sum_{e\in \calN_{\good}}(f(A+e)-f(A))=\Omega(k^*)(f(\calN)-f(A))$---see Lemma \ref{lemma:new-ratio-closed}, Corollary \ref{corollary:new-ratio}, and Lemma \ref{lemma:new-opt}. Thus, the estimate achieves the properties (i) and (ii) mentioned above which leads to the stated competitive ratio. 

The main takeaway from Algorithm \ref{algo:pseudocode-polymatroid} using the estimator $q_t$ given in \eqref{techniques:estimate-q_t} and its analysis is that the online arrival order has sufficient information to achieve an $O(\log^2 r)$-competitive ratio. We will discuss the runtime issue of Algorithm \ref{algo:pseudocode-polymatroid} shortly. We mention that our Algorithm \ref{algo:pseudocode-polymatroid} and its analysis specialized for coverage functions corresponds to the algorithm of Emek, Goldbraikh, and Kantor for \DSC \cite{EGK19}. Thus, one of our contributions is appropriately generalizing their algorithm and analysis from \DSC to the more general case of \DPB.  

Now, we address the runtime of Algorithm \ref{algo:pseudocode-polymatroid}. We observe that the quantity $q_t$ is NP-hard to compute. 
%The problem of computing a min-sized non-empty quotient of a polymatroid is NP-hard. This is because, a min-sized quotient of a matroid is equal to the cogirth of the matroid which is NP-hard to compute \cite{Var97}. It is easy to see that cogirth of a matroid reduces to computing $q_t$ and hence, $q_t$ is NP-hard to compute. 
%For this reason, we believe that the estimate $q_t$ is not likely to be computable in polynomial time. 
%The next issue is how to compute the value of $q_t$ in polynomial time. 
However, we note that a $\text{poly}(r)$-approximation of $q_t$ is sufficient for the desired competitive ratio since our goal is to estimate $k^*$ within a $\text{poly}(r)$ factor. We show that an $r$-approximation of $q_t$ can be computed using a \emph{strength decomposition} with respect to $f_{|\mathcal{N}_t}$. 
%, which is a descending sequence of sets $\mathcal{N}_t=S_0\supseteq S_1\supseteq \ldots \supseteq S_w=\emptyset$. Let $i\in [0,w]$ be the index with $e_t\in S_{i-1}\setminus S_i$. We compute $$\eta_t:=\frac{|\mathcal{N}_t\setminus S_i|}{f(\mathcal{N}_t)-f(S_i)}$$ and prove that it is an $r$-approximation of $q_t$. 
See Algorithm \ref{algo:pseudocode-polymatroid-polynomial} and its analysis in Section~\ref{section:poly-algorithm} which completes the proof of Theorem \ref{main-result:polymatroid}.

Finally, we outline our simpler algorithm for \DCSS and \DST mentioned in Theorem \ref{main-result:hypergaph}. For simplicity, we will focus on \DST here. The polymatroid $f:2^E\rightarrow \Z_{\ge 0}$ of interest here is the rank function of the graphic matroid defined by the undirected graph $G=(V, E)$. Our Algorithm \ref{algo:pseudocode-polymatroid} for this polymatroid can be implemented in polynomial-time since the estimate $q_t$ is equal to the min $u_t$-$v_t$ cut value in the graph $(V, E_t)$ containing all edges that have arrived so far. We recall that min $u_t$-$v_t$ cut can be computed in polynomial time via one application of max flow. However, we show that a much simpler estimator for \DST also achieves properties (i) and (ii) mentioned above: we use 
\[
\eta_t:= \text{number of edges between $u_t$ and $v_t$ in the graph $(V, E_t)$}
\]
where $u_t$ and $v_t$ are the end vertices of the edge $e_t$ that arrives at time $t$. Our proof that this estimator achieves the properties (i) and (ii) mentioned above is via a direct combinatorial argument and it also generalizes to \DCSS. See Section \ref{section:hypergraph-faster-algo} for details. 

%Finally, we consider \DST, which is the special case where $f$ is the rank function of the graphic matroid defined by an undirected graph $G=(V,E)$. Our algorithm mentioned above uses the minimum $u_t-v_t$ cut value in graph $(V,E_t)$ as the estimation of $k^*$ at timestep $t$. Indeed, we can use the number of edges connecting $u_t$ and $v_t$ in graph $(V,E_t)$ as an easier estimation. This new estimation still allows us giving an upper bound on the number of timesteps with too small estimation through combinatorial arguments, which implies a faster randomized online algorithm with the same competitive ratio for \DST. The idea for \DCSS is the same as that for \DST. See Section~\ref{section:hypergraph-faster-algo} for details.
